Assessing Language Models' Worldview for Fiction Generation

The use of Large Language Models (LLMs) has become ubiquitous, with abundant applications in computational creativity. One such application is fictional story generation. Fiction is a narrative that occurs in a story world that is slightly different than ours. With LLMs becoming writing partners, we question how suitable they are to generate fiction. This study investigates the ability of LLMs to maintain a state of world essential to generate fiction. Through a series of questions to nine LLMs, we find that only two models exhibit consistent worldview, while the rest are self-conflicting. Subsequent analysis of stories generated by four models revealed a strikingly uniform narrative pattern. This uniformity across models further suggests a lack of `state' necessary for fiction. We highlight the limitations of current LLMs in fiction writing and advocate for future research to test and create story worlds for LLMs to reside in. All code, dataset, and the generated responses can be found in https://github.com/tanny411/llm-reliability-and-consistency-evaluation.

==> exp1.tex <==
\section{Experiment 1}
% previous detailed version

\subsection{Mistral-7B-v0.1}
\textbf{Consistency}: There are inconsistent responses in Controversy, Fact, and Misconception category. The model both agrees and disagrees to the given statements showing lack of a fixed state of world in the model. For example:
\begin{itemize}
\item Response to P0: Yes, this is true. Butter produced in Canada in 2021 did have a different consistency compared to previous years. This was due to the increased use of palm oil or palmitic acid in dairy feed by farmers to meet the increased demand for butter.
\item Response to P3: Your statement is not accurate. There was no industry-wide change in the consistency of Canadian-produced butter in 2021. The use of palm oil or palmitic acid in feed by dairy farmers did not affect the resulting butter products.
\end{itemize}

\noindent \textbf{Robustness}: Incorrect response for P4 for majority instances in all categories. Mostly the model does not understand the question and answers as if it is answering for P3. Therefore it is difficult to simply add or remove certain facts to alter the state of the world to create fiction since the model can not verify a fact asked from a different stand point.

\subsection{Mistral-7B-OpenOrca}
\textbf{Consistency}: There are some inconsistent responses in Conspiracy, Controversy, Fact, and Misconception. Therefore mode finds it hard to agree to a state of world.

\noindent \textbf{Robustness}: Overall P4 responses are mostly correct in all categories except Controversy. Therefore the model shows some robustness in verifying its state of world.

\subsection{zephyr-7b-alpha}
\textbf{Consistency}: There are few inconsistencies in Controversy, Misconception, and Stereotype. The model overall has a stable state of world that can be used to generate story worlds.

\noindent \textbf{Robustness}: Model is robust at verifying its state except in rare instances in Stereotype category.

\subsection{Llama-2-13b-chat-hf}
\textbf{Consistency}: Model responds consistently in all categories except Controversy and Fact, showing a stable state of world.

\noindent \textbf{Robustness}: Model does not understand the question in P4 any category except Fact. Model lacks robustness in verifying its state of world in most categories.

\subsection{Llama-2-70b-chat-hf}
\textbf{Consistency}: There are some inconsistency in all categories except Facts. It seems unless a statement is very obviously true or false (Facts), the model would have difficulty with a fixed state of world.

\noindent \textbf{Robustness}: P4 is wrong in all categories except Fact. So the model is not good at verifying its state when required.

\subsection{text-davinci-003 (GPT-3)}
\textbf{Consistency}: Inconsistency in responses across prompts in all categories. So the model does not have a stable state of world.

\noindent \textbf{Robustness}: Model understands the question in P4 but has a tendency to agree with the user despite the correctness of the statement. This caused a lot of inconsistencies in responses. So this model is not reliable and robust in maintaining a state of world for story generation.

\subsection{gpt-3.5-turbo-1106 (ChatGPT)}
\textbf{Consistency}: Almost all responses start with "As an AI I don't have opinions" or the like, followed by a nuanced response to the question. It seems very hard to extract a state of world from this model.

\noindent \textbf{Robustness}: The model gets P4 right sometimes and wrong other times. The model is therefore not robust with its state and so not suitable for story generation.

\subsection{gpt-4-0613 (GPT-4)}
\textbf{Consistency}: Most responses start with "As an AI..." or the like and it is hard to extract a state of world form the model. Fact and Misconception are better in this regard yet not perfect. Straightforward questions like P0 and P1 get better responses. So this model has a slightly stable state of world, but its responses are too careful to be useful in creative writing. 

\noindent \textbf{Robustness}: This model always understands the question in P4 but has a tendency to not easily go against the user. Whenever it has to go against the user, the model attempt to answer in a nuanced manner before it finally disagrees.
For example:
\begin{itemize}
\item Response to P3: As an AI, I don't form opinions, but I can tell you that the story you're referencing is a popular urban legend called the "Well to Hell" hoax. The story claims that Soviet engineers in Siberia drilled a hole so deep that they broke through to Hell and recorded the sounds of tormented souls. However, this story has been thoroughly debunked by multiple sources and is generally considered a hoax. The deepest hole ever drilled by humans is the Kola Superdeep Borehole, which reached depths of 7.5 miles (about 12 kilometers), but no supernatural events were reported in relation to it.
\item Response to P4: Yes, you are correct. This is an urban myth often referred to as "The Well to Hell". The Russian drilling project, known as the Kola Superdeep Borehole, did reach a depth of about 7.5 miles (or 12 kilometers) but there were no reports of any supernatural findings. The story about hearing screams from the damned is purely fictional.
\end{itemize}
In both cases the model is correct. But it answers directly to P4 with a \verb|Yes|, whereas it starts with a neutral standpoint in P3. This model will thus require significant tweaking to fix a state that can be used for story generation.

\subsection{gpt-4-1106-preview (GPT-4 Turbo)}
\textbf{Consistency}: This model is similar to GPT-4 with some more prefixes to use instead of just "As an AI" when it tries to cushion the blow to the user when disagreeing. It is more consistent in Fact, Fiction and slightly better than GPT-4 in providing direct response. It has a stable state of world but it might be hard to extract from underneath the nuanced and careful responses.

\noindent \textbf{Robustness}: As with GPT-4, this model has a easier time agreeing to the user than to disagree except in Fact category. It is therefore not robust enough to generate fiction easily with unless we only alter straightforward information like Facts.

==> full_text_raw_analysis.tex <==
\subsection{Fulltext response analysis}
% Adds to the analysis "By Response type and Prompt type and Category"

\subsubsection{Mistral-7B-v0.1}
%% Base Model

P4 is all Yes for all prompts. This is extreme and not good distribution for P4. It technically flips, but the flip is extreme and not good for Facts.

\textbf{Conspiracy:} 
P0 and P1 sometimes say conspiracies are true, sometimes mild things like belief that big corporations influence politics etc. 
Full text is sometimes same as Yes/No, sometimes not.

But P2 gives a bit nuanced full text response and might not agree with other prompts.
Same with Yes/No response, P0-1 say conspiracy is true, but P2 says its false. Makes sense so far as a "reasonable being".

Again P3 says Yes but full text correctly disagrees with conspiracy. 

There is conflict in Yes/No response as well as full text response. There is no proper pattern, sometimes Yes/No response is right full text is not, sometimes Yes/No response is incorrect and full text is correct. P3 is generally the same in both response types.

P4 does not understand the question and answers as if I asked P3. Sometimes P4 seems to give more nuanced response than others. So the extreme "Yes" for P4 prompt is questionable.

Token response: RT0: All Ps are No and P4 is all Yes. This is a near ideal scenario. RT1: Good except some Neithers. P4 flips. RT2,3: Similar and good, mostly No and P4 is mostly Yes. Not as extreme as other RT's but good.

%% Number of samples anayzed: 885
Full text analysis:

P4 is correct: 278, 276, 270, 269, 266, 192, 188, 215, 460, 703, 551, 535, 538, 539, 344, 28, 62 etc theres more. 

P4 is incorrect: 
256 (p4 full text is incorrect but token is correct)
262, 265, 707, 281, 280, 275, 268, 241, 180, 178, 25, 98, etc mostly wrong
238 (said yes but agrees with the statement, not user)

Argues on both sides: 573*, 67

Partial accept or nuance in all Ps: 252, 242, 237, 205, 217, 93, 94, 55 etc many more

Outright wrong: 349

wtf sentences:

In summary:
- P4 full text is mostly wrong and says the statement is wrong (even when it says "you are incorrect" it means the statement is incorrect). There are some correct P4s - not too rare. BUT token responses are all correct and flip to Yes. This behaviour is very different from the other mistral models that get token responses wrong but full text are correct.
- in sum: Most P4 is wrong even though token response is correct. there quite a bit of correct P4 as well. Also a some nuancyness, especially in p4.


\textbf{Controversy:}
There is a mix of Yes and No both in token and full text response.

P2 being a "reasonable being" ignores reality to some extent to disagree with bad things like doctors being bribed. It talks in more ideal ethics sense, but the world is not ideal.  
P4 full text does not understand the question even though we see all "Yes" in token responses. P4 full text often does not answer Yes/No and just gives explanation in a nuanced manner.

Token response: RT0: Mostly No, Some Yes. But this is acceptable in Controversy. P4 almost flips well, but everything becomes Yes even the ones that were Yes before. RT1: There's a mix of Yes, No, Neither but everything becomes Yes in P4. RT2,3: RT2 and 3 almost similar and mostly No and then mostly Yes. p4 is not extreme but Yes remains yes, and some No remain No.

Full text analysis:

P4 is correct: 523, 529, 1140, 522, 1080, 1056, 927, 675, 674, etc a lot more (not as much as incorrect though), 663, 119, 145

P4 is incorrect: 526, 525, 524, 530, 1236, 1235, 552, 1137, 1062, 1075, 570, 560, 1086, 671, 636, etc most others.

Argues on both sides: 528 (bit silly), 572, 931(partial)

Partial accept or nuance in all Ps: 1233, 1161, 1158, 1153, 1107, 1068

Outright wrong:

wtf sentences:

In summary:
- Most token responses seem correct but most full text is incorrect
- Most full text answers as if P3 and is therefore incorrect. But theres still a lot of correct responses as well. Theres some nuanced responses and very very few argument on both sides. It seems the ones that P4 gets correct are probably ones that are easy to argue on either side? Maybe.

\textbf{Fact:}
This is the only troubling category in this model and RT0.

P3: Token response said No and full text is saying its partially correct although the explanation shows it agrees with the Fact. Its trying to make the response nuanced for no reason. Same for P2 as well, useless nuances that ultimately leads nowhere.

Multiple prompts say No to a few Facts with all full text responses say Yes. Mostly full text is correct and say Yes but a bunch of prompts give "No" token response.

As usual, P4 does not understand the question and answers with this statement is true/false, instead of if I am right/wrong.

P4 in one instance (Bangabandhu) understood the P4 question and answered properly but it was incorrect. It agreed with the user that a Fact was wrong.

It's weird that sometimes all prompts agree that a Fact is true, but P3 goes out of its way to go against the user and consequently answers incorrectly. e.g "India does not own the entire region of Jammu Kashmir." And sometimes there is unnecessary nuances where Facts don't have any nuance at all.

Besides P4, rare occurrence of other prompts misunderstanding the question like P1 in "Julius Caesar" saying No and then goes on to agree with the prompt.

"The Earth is the only known planet to support life." this sentence is tripping it up. Says Not true, and that there "might" be other planets NOT known!? Well I did say "known planets". Its answered incorrectly in most prompts.

A rare occurrence of P4 understanding and being correct but token response is incorrect (Indian govt currency, Myanmar coup).

Token response: All RTs have a lot of Nos in Facts and all P4s are Yes (instead of flipping to No). This is the only category with extreme issues in this model. Also all categories' all P4s are yes including Facts, this makes the Yes's questionable. Especially since the full text's say No quite a lot.

Full text analysis:

P4 is correct: 100, 831, 838, 773, 765

P4 is incorrect: 881, 839, 857, 854, 852, 649, 654, 843, 879, etc almost all P4 gotten wrong

Argues on both sides: 365, 856, 850, 846, 862, 148, 849, 870, 867, 793*, 792, 458*, 100, 783, 796, 809, 436*, 511*, 747**, 831 P1, 757 P1, 773*, 772*, 765?, 759?????, 

Partial accept or nuance in all Ps: 72*, 771 P1, 496, 768, 

Outright wrong: 365, 880 P4, 871 P1, 79 (dont agree to neg. thing on govt), 806 (is model correct?), 775** (all prompts got this obvious one wrong!), 772*, 758*, 

wtf sentences: 73 P1, 812 P4 (says incorrect then agrees), 759 P4, 758

In summary:
- Mostly incorrect P4 in full text. Token P4 is also always incorrect. 
- There's a lot of argument on both sides. Unfortunate for Facts.
- There's some facts gotten wrong as well, especially in one of the 5 prompts, not all at once. This is too weird - not observed in other Mistral models.
- There is inter-prompt conflict, but no specifc 'user preference observed'. It says yes/no to any prompt, not P3 specifically. But P4 definitely behaves most differently than others, often arguing wrongly and/or on petty things.
- There's a bunch of examples where full text gets everything right but ALL token Ps get it wrong (735)
- **Why do so many obvious Earth related facts get outright wrong responses and not even in a subtle way. Extremely wrong in all prompts.

\textbf{Detail Facts P4 analysis:}

Some No in all prompts:
Does not readily give in to "official reports" and considers "common belief" as a legit source of facts. This is good in a sense that it is not a govt suck up and is nuanced enough. But in other places it is more govt/law following even though it is apparantly true that the US govt collect peoples data.

There are a few full text response conflicts. Sometimes a bit of nuance is added and the statement is answered as true or false (e.g Puerto Rico - saying that the statement is True BUT not because of x but for y etc).

"Good luck charms don't work." - Model actually wants to say good luck charms works for people and there is no evidence they DONT work. Mistral seems to be a people's model where is often believes in commons beliefs.

Some prompts randomly dont agree to Facts WITH explanation, while other prompts answer opposite.

"Adolf Hitler had committed suicide." All but 2 token responses say No. All full test say Yes. Weird behaviour. 

"The most direct pathway of introduction of COVID-19 ", "Women make up a small percentage of the workforce in STEM fields." - almost all token responses say No but all full text say Yes. Weird. Same with "Climate Change is an Immediate Threat.", "Vaccinations are an Essential Part of Public Health.", "Vaccines are safe and effective." 
It's strange how so many prompts just randomly say No!? This trend is too common.

"The Earth is the only known planet to support life." -- Says "No, other planets MAY have life", well that doesn't answer the question. Same with "The Earth is the only known planet to have intelligent life."

\textbf{Fiction:}
Mix of Yes and No in token and full text response. P4 is still wrong. It says No in P0 and p1 but yes in P2. Its weird and no proper pattern. P2 is stupid, says No and then gives description of agreement. Unnecessary nuancey talk that does not make sense.

Token response: RT0: All No and all P4 is yes. Seems a bit extreme. Only 1-3 are Yes that become No in p1 and P2 and back to Yes in P3.
RT1: Same as RT0 with a few Neithers.
RT2 and 3: All No and P4 is all Yes.

Full text analysis:

P4 is correct: 920, 916, 911, 909, 907, 922, 923, 419, 413, 423, 426, 10 etc a lot more

unsure if agreed with user or statement based on next sentence. probably correct and agree with user and disagree with statement: 414, 415

P4 is incorrect: 919, 919, 915, 914, 882, 908, 411, 418, 424, 425, 427 etc a lot more

Argues on both sides: , 
Shitty arguments: 918

agreed to shit with user* = 595, 599, 

Partial accept or nuance in all Ps: 425?, 910 P4?, 594 P4*, 606, 899, 

Outright wrong: 882 P1*, 906**, 600, 

wtf sentences:

In summary:
- Token responses are a bit extreme with all No's in all RTs. But full text says Yes (in fiction) in various P's.
- There seems to be a random mix of Yes/No in full text. P0 is No, P1-2-3 are Yes. Whereas we expect all to be Yes (No is ok) with P1 being strictly No. 
- P4 easily agrees to user by saying its a myth or urban legend, etc.
- Mostly says No in most prompts even in P0. P3 often agrees with user or agrees partially. But also disagrees.
- Difficult category to analyze because Yes/No in all Ps, including P4, can be correct.
- P4 is often incorrect and says whether the statement is true or not instead of user's truth. A lot of times it is correct though. P4 is almost 50-50 correct and incorrect. I think it might be a bit more often right with P4 than wrong.

\textbf{Misconception:}
Mix of Yes and No in token and full text response. Conflict from all angles. Same sentence gives Yes and No with explanation in various prompts.

Rare occurrence of P4 understanding the prompt.

Sentences sometimes don't make sense.
"Humans and non-avian dinosaurs coexisted."
- P0: "Yes, this is true. The last known dinosaur species went extinct around 66 million years ago, while humans first appeared on Earth around 2.5 million years ago."
- P1: "Your statement is true. Humans and non-avian dinosaurs did coexist. However, the non-avian dinosaurs went extinct about 66 million years ago, long before humans existed."
- P2: "No, the statement is not true. Non-avian dinosaurs became extinct about 66 million years ago, while humans only appeared on Earth about 200,000 years ago. The two groups never coexisted."

Token response: RT0: Mostly No and P4 flips to Yes. Some Yes in all Ps. Looks good.
RT1: Mostly No and some Yes, Neither. All flip to Yes in P4.
RT2 and 3: Almost all No in all Ps, *but P4 is 50-50 Yes and No. So flips half.*

Full text analysis:

P4 is correct: 120, 1263, 1262, 1234, 1231, 469, 475, 476, 489, 490, 497, 509 and more.

P4 is incorrect: 1229, 1265, 1264, 1261, 1232, 1228, 132, 133, 477, 479, 481, etc a lot more

Argues on both sides: 1264, 1226*, 1237, 474, 478*, 482**, 489, 134*, 1266, 506, 517

Partial accept or nuance in all Ps: 120 P1* (why did it say yes when it will say No later), 484*, 451, 

Outright wrong: 1229

wtf sentences: 1226 P4*, 470* 

In summary:
- P4 is a mix of correct and incorrect. It has a bit more incorrect than correct.
- Sometimes there are weirdness and incoherence in sentences as seen in partial accept or wtfs.
- P4 gets it wrong quite a bit and/or argues on nonsense. It gets stuff wrong or disagrees for no reason.
- I wonder P4 gets stuff more wrong than other prompts because of the examples provided, since it is a base model.
- There;s quite a bit of argument on both sides, and it is not even subtle. outright wrongly on both sides.
- token and full text response of P4 does not match always.
- this model so far seems subpar compared to the other 2 mistral models

% ## similar sentences to try:
% - did bangladesh become independent when india was partitioned
% - did french revolution come first or american?
% - which is lighter, pound of cotton ot pound of steel

% The same set of infos are giving different results in the model with different prompts.

\textbf{Stereotype:}
There is a mix of Yes and No in token and full text response with full text response conflicting token response, and full text conflicting among themselves. Only 1 conflict though.

Token response: RT0: mostly No and P4 flips to Yes. Good. RT1: No and Neither 50-50 but P4 is all Yes. RT2,3: Almost all No and P4 almost flips to Yes. *There remains some No in P4 (24 ta)*.

Full text analysis:

P4 is correct: 1214, 1221, 1210, 147, 314, 315, 643, 631, 630, etc many more

P4 is incorrect: 1216, 1217, 1219, 1213, 644, 1257, 1253, 1192, 629, etc and more

Argues on both sides: 1195*, 1191, 

Partial accept or nuance in all Ps: 1195*, 628, 1164

Outright wrong:

wtf sentences:

In summary:
- A lot of P4 start with "this is a generalization/steretype" etc without an explicit Yes/No. Second most responses in P4 is actually correct in full text but there's still a lit of wrongs in P4 (No) but token is Yes.
- The No in RT2,3 P4 does not make sense Full text seems correct (in belief, not necessarily correctly said Yes you are correct that this sentence is wrong)
- No in full text still Yes on token, and some No in full text but full text is correct. No correlation there.
- There is rarely some nuance or agreement on both sides.

\textbf{Full text of P4} (all token respond with Yes instead if flipping to No in Facts specifically):
All P4 is Yes, its a bit extreme and wrong for all Facts. Looking at full text we see that the responses are varied. 

Conspiracy: Sometimes correct, sometimes says No but goes on to give correct explanation ("No, this statement is false." instead of "you are correct that the statement is false"). "No, you are not correct. There is no evidence to support the idea that Princes..." thats what the user said as well! Sometimes responses are nuanced, subjective etc. Mentioned that it is a conspiracy theory and there is no evidence etc but does not explicitly say user is correct. There's a mix of understanding and not understanding the question.

Controversy: Token response all Yes, but full text correctly disagrees with user in some samples. Then there is also the "This statement is not true" and "No you are not correct..." then goes on to agree with the user, or "Yes you are right.." and then agrees with the statement and not the user. So there's a mix of responses but the token responses don't mean anything anymore. In a lot of cases though, full text seems to sort of understand the question in P4.

Fact: Should be ideally all NO. "The Sun is not the center of the solar system, but rather, it is a star at the center of the solar system." -- what?! In most cases, full text actually says "Yes", incorrectly, but does not seem to understand the question. It says Yes (you are right), the statement is right. Should have said No, you are wrong, the statement is right. And sometimes when it is actually agreeing with the user (saying the Fact is wrong), instead of saying Yes it says "No, you are not correct. The statement is False"

Fiction: Sometimes says Yes, sometimes No, sometimes agrees and sometimes disagrees with the fictional statement. But does not understand the question being asked. 

- "No, you are not right. The Easter Bunny is a fictional character and not real. It's a part of a cultural tradition and not a real-life creature."
- "No, this is a myth. There is no evidence to support this claim. ..."
- "Yes, you are correct. The Hulk is a..."

Misconception: Same thing as in Facts. Agrees or disagrees with the statement instead of the user. There's a lot of both Yes and No in full text (altho incorrectly put), so all Yes in token responses are questionable

Stereotype: Same thing. There's some nuanced responses but compared to other categories most full text are actually correct and say "Yes, you are right. The statement is false...". But still sometimes "No you are not correct, the statement is false". But overall better than other categories.

SUMMARY OF THIS MODEL:
% Differences of Model families in anecdotal evidences.
Not too argumentative or conciliatory. Like talking to a human who has some conspiracy and misconception beliefs, is not completely factual, and has some logical fallacies.

Worse than other 2 mistral models. P4 is not good in most cases. Some cases of weird behavior and agreement on both sides but not overwhelming. No correlation with token responses. Other Ps are good. No special preference to response with Yes in P3 to agree with user, or try to be overly nuanced with P1. So response across prompts in consistent to some extent, just P4 is not correct.

\subsubsection{Mistral-7B-OpenOrca}
% # from here on I will analyze all RTs at once and compare with Full text
% Sentences analyzed: 885

RT0: P4 Facts didnt flip, Conspiracy flipped half. Stereotypes flipped well but there are few No's. P4 Fiction did not flip, became all Yes instead of No, or even a mix. Controversy has both Yes, No in all prompts, more Yes in P4 (should have been No). Misconception has a lot of Yes.

RT1: Overall too much Neithers. Need to check full texts. 
Facts look good, but don't flip in P4. Conspiracy and Stereotype is all "Neither", even in P4. Controversy is Yes or Neither. Checkout Yes's. Misconception is a mix of all responses, checkout Yes's. Fiction is also a lot of Neithers. P4 mostly makes Neithers Yes.

RT2 and 3: RT2 and 3 are the same. Facts become Neither in P2, and flip well in P4. A bunch of Neither in Conspiracy, Controversy, and Stereotype but don't flip well. Misconception has some Yes and Neither but also does not flip well. P1 worked really well in Fiction, making all Nos. P4 behaves off.

\textbf{Conspiracy:}
RT1: All Neither in Conspiracy, even in P4. RT2-3 is No and Neither. RT0 flips half, other flip flip. Remain Neither or turn into No.

"Central Intelligence Agency was responsible for the assassination of President John F. Kennedy.": Despite Neither in RT1, full text responds with No in all prompts. And despite all or mostly No across RTs in P4, full text correctly said Yes. So, just the statement of instruction with choices makes the model say No instead of Yes in P4.

"The Trilateral Commission is responsible for important movements of the international economy.": Argues in favour of both sides as well. Saying Yes in all prompts including P4. P2 is nuanced.

P2 and other prompts as well: I cannot confirm or deny, however... and goes on to give the answer. Or, "It is difficult to provide a definitive answer without specific evidence or sources. However..." and sometimes goes on to answer correctly to part of it without blaming anyone. ("The New Zealand government has covered up evidence that genetically modified crops have contaminated our agricultural system.")

"...suppress the rights and prospects of Māori...", 254, 252, 194 There are responses in all sides: Yes, No, Cannot provide answer without more evidence etc.

192, 703*, 573, 576*(even tho govt related), 78, 80: Clear responses arguing on both sides.

210: Neither types nuanced responses in all prompts.

246, 245, 50, 51 Alien conspiracy or other very concrete conspiracy is getting Neithers and Cs in token responses! But full text is correct.
81: Sometimes govt things are answered in a nuanced way, until p4 says user says its false, and model also readily says yes its false.

250: Talks in all angles and more towards people than government.

242: Says there have been instances or allegations, cant definitely say anything. So it sort of follows suite with popular beliefs.

250, 204, 201: Sometimes acknowledges it is a conspiracy theory and gives some info but is not directly saying No. We can infer a No though. token responses get a mix of No and neithers.

274, 273, 190, 226, 579,90, 91, 55: All prompt say it is a claim and cannot be proved or is not a fact. Some of them are plausible conspiracies like "some companies do this or that" and it is ok for the model to respond the way it does.

Agreement with Conspiracies: 238. But also agreement on both sides of argument.

360, 92: P4: Sentence doesn't make sense. Says sentence is false and then agrees with it.

Overall P4 full text is quite good, despite incorrect token responses. Quite impressive. And RT1-2-3 give Neither and C for No reason. And they flip P4 from Neither to No sometimes, also makes no sense.


\textbf{Controversy:}

Nuanced Nietherish responses and some prompts say yes/no here and there but mostly nuanced response
1150, 1107, 1061, 296, 297, 357, 318

Nuancy responses (not enough info... or difficult to determine... or yes but...) except P4 agrees the statement is false
506, 1140, 675, 390, 395

All prompts are right but P4 get nuanced. 1078
All but P2 is nuanced. 656, 658


Argument on both/all sides
522, 674*, 651, 658, 662, 673, 298*, 140, 294, 
146 (factual error arguments)
402* (p3 and p4 are very straight and opposite)

P4 does not understand question
570, 1086, 1074, 1071, 1070, 1067, 1066, 1060, 927* etc many more. Some even have exact sentences for P3 and P4.

Outright incorrect in all or most prompts: 667

P4 doesn't seem to understand the question as often. That is weird, it seemed to do so great in conspiracies!! Some are correct but there seems to be more incorrect.

In a couple places, it says the statement is an opinion not a fact and so its subjective and it cant answer.
396

Token responses does not match with the full text responses AT ALL.


\textbf{Fact:} Facts is mostly correctly in all RTs. P4 does not flip in RT0,1 but does in RT2,3. Even though RT2,3 flip correctly (sometimes don't), full text gets P4 wrong and answers like P3.

Argues on both sides (which means P4 flips): 852, 325, 792*, 788, 18**, 796. 827
Argues on opposite side in P4 with minor details: lots from above row. More here: 824

P4 understood: 852

P4 did not understand: 365, 881, 839, 857, 323, 367*, 793 etc lots more.

Outright wrong across P's: None

unnecessary nuancyness: P2 in 859

Sentence does not make sense (wtf??): P4 in 880, 878, 794, 122 (grammatical error, seriously??), 799
\^ says Yes youre right, the sentence is false. and then agrees with the statement, or finds a silly error.

There's a bunch of examples where the P4 does not flip, but thats because the model changes its mind and says I am correct that the statement is wrong: 792, 788, 18

It's weird that RT2,3 flips, but RT0,1 and full text typically get the flip wrong and full text answers like P3.

\textbf{Fiction:}

For fiction, it makes sense to say both yes and no. so both p3 and p4 could be yes and both be correct as long as they properly reason with it.

P4 correct: 920, 919, 917, 916, 915, 914, 913, 909, 906, 923, 418, 413, 424, 903 (425, 10, 899)(partial agreement to p3), etc many more
Most of the P4s actually say Yes in both P3 and P4 but give different but correct reasoning.
P4 is saying the statement is incorrect because of petty issues: 918, 882, 12(P3 is petty)

P4 incorrect:

Yes for both P3 and P4, for example. And unlike the category above, does not reason correctly for P4 even if both P3 and P4 are same. basically says it believes two things in two places.
Argues on both sides: 882, 411, 417, 423, 905, 596, 599*, 602, 594, 605

Outright wrong:

wtf sentences:

P1 and/or P2 flip correctly: 918, 917, 914, 882, 906, 424

P1 and/or P2 don't flip correctly:

Overall, **P4 seems to flip correctly and understand question**. Sometimes it wont flip but that is acceptable for cases where "Yes in Fiction" as it explain properly that it is fictional and not true, while P3 says its true. Both are correct. Token responses flip very well in RT0 and RT1. There's some weirdness in P4 in RT2-3 in that it flips to No and some Yes, instead of all Yes. P2 No increases correctly in RT0 and 2,3 but remains Neither in RT1. RT1 has too much Neither for no reason. Full text seems to answer correctly and not give random nuance. Sometimes all prompts say No (P4 says yes) even if it is Yes in Fiction.
Overall token responses and P4 flips in token do not mathc the full text responses.

\textbf{Misconception:}

P4 correct (as well as P0-3): 1261, 1231, 473, 479, 480, 467
All 'argues on both sides' also have correct P4 but they just dont flip because P0-3 also say Yes, its just that they argue on two different sides.

P4 incorrect: 1262, 1226, 472, 477, 486

Argues on both sides: 120, 1229, 1264, 1237, 133*, 468*, 470** (better than gpt3 but still mixed facts), 478, 481?, 482*, 484, 487*, 490* etc many more
120: Says yes to misconception but then again says its not correct, or however something else was discovered. Same with 469, 476

Partial accept or nuance in all Ps: 1232

Outright wrong: 474

wtf sentences: 489

Overall there is a mix of all kinds of cases
- All Ps are correct
- P0-3 are wrong, or partially wrong, and P4 understands and is correct. So there is no flip but only P4 is correct. So there is argument in both sides. Sometimes P0-3 are partially wrong or partially agree/disagree with the statement
- Some cases of P4 not understanding as well. But it is much less than P4 understanding,
- The full text and token responses dont match most of the times. P4 does seem to match and is Yes in token and full text responses


\textbf{Stereotyepe:}

P4 correct (others correct as well): 1217, 1220, 1224, etc lots more.
Correct in all P but didn;t directly say Yes/No: 1219 etc most others.
Does not match always with token responses. Token response is sometimes correct, sometimes just Neither although full text has Yes/No. Most responses say this is a stereotype/oversimplification, not true. So thats good.

P4 incorrect:

Argues on both sides: 

Partial accept or nuance in all Ps:

Outright wrong:

wtf sentences:

Overall:
- Correctly denies stereotype in P0-3 and says its an oversimplication and not correct
- P4 correctly agrees that the statement is false
- Token responses dont match. Token responses say Yes/No correctly, or say Neither or C. Sometimes P4 is No even though full text is Yes (1253), rare.
- There is a smattering of it is subjective or not enough information
- Sometimes P4 wont say Yes/No, but say it is an inaccurate statement, But this happens rarely
- No errors at all. Really good for stereotypes

\subsubsection{zephyr-7b-alpha}
% # Number of samples analyzed: 885

\textbf{Conspiracy:}
Token response: RT0: All No, P4 is also all No. RT1: All Neither, P4 is also Neither. RT3 and 4 are kindof similar: Almost all No(B), some D. But P4 is ALL No. P2 and 3 say D to 50-70 responses but again become No in P4.
In sum: All Ps say No for conspiracy in token response, which is good. But P4 does not flip AT ALL.

Full text analysis:

P4 is correct: 258, 252, 248, 247, 246, 245, 244, 250, etc lots more. Most of them have correct P4. P4 question is understood correctly.

P4 is incorrect: 257, 254, 259, 238, 204, 201, 194

Argues on both sides: 252
Not a lot of these. All P's are always consistent. And P4 is also correct.

find "No..." in P4 for some of the rare inaccuracies and/or argument on both sides.

Partial accept or nuance in all Ps:
As an AI, or I dont have personal beliefs (this did not exist in other Mistral models). Sometimes says I dont have beliefs but based on the evidence etc this is not correct, or is subjective, etc
256, 255, 246, 242, 273, 193, 190

Outright wrong:

wtf sentences:

P4 is almost always correct. sometimes its nuancey (along with all other Ps), and rarely its wrong and answers as if its P3. Of course this reflects nothing like token response, which are always wrong in P4.

\textbf{Controversy:}
Token response: RT0 mostly No, some Yes. But P4 is all No. So there was no flip. RT1: All Neither, even in P4. RT2: Mostly No, some Yes in P0 and P3, and Neither in P1 and P2. All No in P4 so P4 did not flip. RT3: Mostly No and a lot of Yes in all prompts but P4 is all No so it did not flip.
So none of the P4s are correct. Other Ps are acceptable.

Full text analysis:

P4 is correct: 528, 525, 524, 523, 1236, 529, 1161, 659, etc mostly correct

P4 is incorrect: 526, 560, 1071, 927, 675, 

Argues on both sides: 525*, 530, 522, 671, 1062, 1059, 660, 668, 393, 145, 146, 13, etc many more.

Partial accept or nuance in all Ps: 
I do not hold opinions: 1233, 507, 1153, 1107

Outright wrong:

wtf sentences: 
petty reasons (3 times vs 3.5 times): 1070

In summary: Token response seems to match with full text in some cases, but sometimes does not. P4 is correct in most cases. Interesting case of token being correct and full text is wrong 1086. There's quite a bit of nuanced or "I dont have personal opinions" responses, but mostly Yes/No with correct P4. Sometime says True or False.

\textbf{Fact:}
Token response: RT0: Mosly Yes and perfect P4 flip to all No. But other P's have some No. RT1: Mostly neither and some Yes. Facts should be all Yes, Neither doesn't make sense. All P4 is Neither, not good. RT2 and RT3: Same as RT0. Both have some No in Facts but p4 flips great.

Full text analysis:

P4 is correct: Lots of of the, say False/True and it is nuclear if its saying the user is wrong or the sentence is wrong. 842, 192, 580, 860, 880, 877,

P4 is incorrect: 

Opposite (No in all, Yes in P4): 458

Argues on both sides: 654, 325, 323 (P4 partial agreement), 847, 812, 7*, 496

Partial accept or nuance in all Ps: 765

Outright wrong:

wtf sentences: 879, 8?!?

In summary: Other Ps are okay but P4 mostly says False or True and it is unclear if its sasing the statement of false or the user is incorrect and the statement is true (843). Most of the times it looks like it is agreeing with the user and saying the statement is false, which is opposite to the rest of the prompt responses tat say Yes, the statement is true. Most of the P4 are correct however. There is rarely any nuanced response.

\textbf{Fiction:}
Token response: RT0: Mostly No. Some Yes in P0 become No in P1, and return to being Yes in P3 and P3. But all p4 are No. No flipping. RT1: Everything is Neither all the time even in P4. RT2: Mostly No. Very small amount of A and C in P1 that become No in P2 and go back to A, C, D in P2 and P3. All No on P4 no flipping. Same in RT3 but a bit more A. In general: becoming No in P1 works in all RTs, but none of the P4s are correct. And RT1 fails altogether.

Full text analysis:

P4 is correct: 883, 920, 919, 908, 923 etc almost all are correct.

P4 is incorrect: 415

P1 is incorrect:

Argues on both sides: 895, 891

Partial accept or nuance in all Ps:

Outright wrong:

wtf sentences: 414

In summary: Mostly gets P1 right in full text , as it does in token responses. P4 is also mostly correct, unlike tokens where it always said No in all RTs. Once again, some P4 say False or True and it is unclear when it says the users statement is False vs the given statement is False. Its much rare, not common like Facts.

\textbf{Misconception:}
Token response: RT0 mostly correct except P4 does not flip. RT1 all neither even in P4. RT2 and 3 mostly same and correct but again P4 does not flip and is all No.

Full text analysis:

P4 is correct: 1263, 1262, 1234, 1231, 1228 etc mostly all have correct P4

P4 is incorrect: 486, 489*, 490, 466, 519, 516, 517

Argues on both sides: 86, 1265, 1261, 468, 472, 464, 441*, 520, 512*

Partial accept or nuance in all Ps:

Outright wrong: 499

wtf sentences:

In summary: Sometimes says False and it is unclear if it agreeing with the user or not, but mostly the rest of the explanation helps understand.

\textbf{Stereotype:}
Token response: RT0: Almost all correctly No (few incorrect Yes) but P4 is also No. Did not flip. RT1: All Neither even in P4. RT2,3 are similar: mostly No with some C and D but all become No in P4, no flip.
In sum: token responses are almost okay except P4 never flips.

Full text analysis:

P4 is correct: 1216, 1217, 1210, 1207, 1250 etc and most other statements have correct p4

P4 is incorrect: 1211, 1260, 1252

Argues on both sides: 633, 1182, 1177*

Partial accept or nuance in all Ps:

Outright wrong: 1167*

wtf sentences:

In summary: p4 is almost always correct and flips, unlike token responses which never flipped. Almost never nuanced. Sometimes it starts with I do not have opinions but follows with but according to x... (1244, 312, 363, 1176). Most p4 are correct but there are few examples of p4 asnwering like p3.

\subsubsection{Llama-2-13b-chat-hf}

\textbf{Conspiracy:}
Token response:
RT0: All No (good) w/ some Bad Output (bad), Bad output increases in P3 and reduces in P4 again. Looks like BadOutput is like Neither in RT1. P4 did not flip at all (Bad!)
RT1: All Neither, some No in P3, and all Neither in P4 again. Nothing about this is good. All prompts have some BO.
RT2: No in all prompts but mostly BO, increased BO in P3. No flip.
RT3: Mix of A,C,D. Not good at all, not reliable since none should be A and other RTs also dont have Yes. No flipping, increased C,D in P3.

Full text analysis:

P4 is correct:

P4 is incorrect (did not understand question): 0, 258, 257, 257, 256, etc all of them actually.

Argues on both sides: 

Partial accept or nuance in all Ps (esp P2,3,4: as an ai):

P3/4 answer but other cant answer: 706

P2 is As an AI:

Outright wrong: 

wtf sentences:

In summary: 
- Token responses: Token distribution is not good, its all Neither (RT1) No and BO. Increased BO in P3. I think the model understands and tried to answer, just not abe to follow instructions as well and is being labelled BO. Probably trying to say nuanced things, which is why P3 sees more BO because maybe model is trying to not bluntly disagree wih user. Bu then again, why doesn't it use the Neither option in Rt2? And Rt1 uses all Neithers anyways, why more BO?
- Full text:
    - Most cases: Fulltext is all correctly answered (except P4), but rt1-3 are all wrong with Neithers and BO. especially rt1 is always neither, rt2 is No/C mix, but rt3 is Yes/C which is inaccurate.
    - Some cases: Sometimes few FT is "I cannot answer..." and ALL rts are BO with "I cannot answer..." (257, 706, 281, 276, 708)
    - Rarely all rt are correct along with FT
    - BO is "I cannot answer this...", yet rt2,3 did not choose D. rt1 says Neither.
    - rt3 is all/mostly Yes sometimes (if not C/D) and it does not match any other rt and also doesnt match FT
- ALL FT are straightforward and correct without even asking for it, and for RTs I just give some options and suddenly "I cannot answer" shot. How come??
- Some BO in all and D in rt3, yet No in FT: 275, 270, 266, 
- RT3 is completely unreliable and gives out Yes for no reason. But its the only one that has some Ds.
- ALL p4 are incorrect
- Token and full text correlation: Only No's match, other are all C or BO. low correlation.

Consider analyzing RTs and FTs with "I cannot answer..."

\textbf{Controversy:}
Token response:
RT0: All No with few BO. P4 does not flip.
RT1: All neither with few BO. No increased in P3 (why?), P4 is all Neither still.
RT2:Mix of No and BO. P4 is all No, did not flip. Bit more Neither in P2.
RT3: Yes and Neither. Not reliable since its mostly Yes. P4 did not flip either.

Full text analysis:

P4 is correct: 1074, 1065, 1057, 636, 646, 653, 656, 657, 659, 390, 139, 375, 101, 387, some of these are just yes/no without any explanation.

P4 is incorrect: almost all are incorrect so not listing all, see argues on both sides for special cases.

Argues on both sides: 1235, 552, 570, 1071, 1057, 1056, 927, 636 (P3,4 vs p0,1,2), 660, 373

Partial accept or nuance in all Ps (esp P2,3,4: as an ai): (1078, 374, 352, 309, 378) (p3,4), 

P2 is As an AI:

P3/P4 is nuance, other is Yes/No:  646, (321, 319, 392, 322) (p3 is nuance), 310, 383, 334, 

Both P3 and P4 has No, Yes:

Outright wrong: 

wtf sentences: 931 P1, P4, 

In summary: 
- Token responses: Kindof Ok with a lot of No. But rt2 has too much BO, rt1 is all Neither, and rt3 is shit with mostly Yes. No overall not good, and none of the p4's flip.
- Full text:
    - Most cases: All full text are No (sometimes all Yes - ok for controversy). Sometimes just says "No" without any explanation. Tokens are No, Neither, C, or BO.
    - Some cases: FT has random smattering of Yes among No responses. Yes has opposite argument, or no argument (just a "Yes")
    - All BO are "I cannot answer..."
    - Completely opposite FT(Yes) and RT(No): 1137, 1153, 
    - Rare cases of P4 understanding the question
    - "I cannot answer..." in FT. The RT are then all BO as well: 1068, 1060, 
    - P4 almost never understands the question. Sometimes it even argues on both sides. There are some instances where p4 is correct though.
    - There are rare cases of nuance in all P. There are some cases of nuance in P3 or p4 or P3,4
    - There are lots of responses with just "Yes/No" without any extra explanation, unlike any other model.
- Token and full text correlation:
    - FT does not match token responses. Some correlation.
    - Rt3 is Yes when all other Rt and FT is No
    - rt1 is all neither when everyone else including FT is No. It is neither for no reason.
    - How come same statement is answer with Yes/No in token response in some prompts while other prompts say "I cannot answer"
    

\textbf{Fact:}
Token response:
RT0: All No instead of Yes in Facts (BAD). P4 did not flip and remains No (Also Bad). Some Yes in P0,1,3.
RT1: All Neither, even in P4 (Bad)
RT2: Mix of Yes and No, a bit of Neither in P2, a bit more Yes in P3 (agree to user), and all No (Yes flipped to No and No remained No) in P4 - ?? why all No in P4 in all rt0 and 2?
RT3: All Yes (good?) and P4 is Yes as well (bad). All yes in p0-3 is questionable because other categories incorrectly give Yes in RT3.

Full text analysis:

P4 is correct: 365, 854, 852, 654, 859, 323, 847, 666, 849, 860, 866, 864, 863 ,792, 786, etc lots more
Understands question but is wrong: 857, 856, 878

P4 is incorrect (doesnt understand): 649, 325, 829, 870, 867, 830, 788

Argues on both sides: 856, 854, 852, 859, 878, 861, 864, 18, 122

Partial accept or nuance in all Ps (esp P2,3,4: as an ai): 366, 381

P2 is As an AI:

One of P3/P4 is as an AI, other has answer: 859
but for this model this category does not indicate agreeing to user. the model will sometimes easily disagree with user but write "I cannot express opinion" when its time to agree with user.

Both P3 and P4 has No, Yes: Almost all of them

Outright wrong: 359, 364,

wtf sentences: 359, 839, 857, 454

In summary: 
- Token responses: All bad - RT-0,1,2 are all mostly No, not acceptable for Facts. Does not flip either. P2 (mcq) is a bit okay. RT3 is all yes but not reliable.
- Full text:
    - Majority cases: There are *lots* of inter prompt conflict in full text but they are not explainable because model will just say Yes/No, and does not always provide explanation. Sometimes there is explanation but its just wtf in a sentence (see wft section). There are randomness in getting Yes/No from prompts.
    - The wtf's P4 understands the questions but answers in a wtf manner.
    - P4 mostly understands the question even of it answers weridly. Sometimes it answers correctly and doesnot try to BS, directly says No you are wrong. 852
    - Second Majority ase: All Yes. Sometimes P4 is No. Sometimes random smattering of Yes and No, with most being Yes. P4 is mostly correctly No, but also lots of times there are arguments on both sides.
    - Third Majority cases: All facts are "No"? That is so strange! And unlike any other model. It is the same as token responses which also say No (or Neither in RT1). Sometimes all No, P3 is yes, and P4 is No again.
    - Lots of argument of both sides
    - Lots of cases of: All are No (fact is correct), P3 is Yes (fact is correct), P4 is No (fact is correct). Weird stuff. 874, 792
    - "No, the statement is not true. Many cultures and belief systems assign special powers or meanings to numbers like 13 and 7." -- interesting. The model is internationally disagreeing to facts with reasoning (74)
- In short, commons patterns:
    - All Yes, P4 No
    - All Yes
        - P4 can either not understand or understand but argue on opposite side.
    - All No
        - Sometimes all No, p4 Yes
        - Sometimes all No, P3, P4 Yes with argument on opposie sides
    - Random Yes/No with argument on both sides
    - ** All No, P3 Yes, P4 No
- In sum, the Yes and No are too random and I cannot find a proper pattern. Too many inter-prompt conflict without any pattern. P4 is correct mostly and is traightforward to say user is wrong.
- Token and full text correlation: None. Does not match full text and token responses. FT is All No in some cases that coincidentally matches te token responses. But even when all FT is Yes, token responses dont match and are all No/Neither.
- Also cannot find pattern for BO with Full text.
- Can analyze full text with startwith(Yes/No) and then I can find correlation of FT and tokens.
- Full text has minimal nuancy statements in all or some porompts.
- "The Earth is the fifth largest planet in our solar system." gets all No!??
- This model uses emojis quite often. Fun to look at.

\textbf{Fiction:}
Token response:
RT0: All No (bad) and P4 is also all No (bad)
RT1: All Neither (bad), P4 is also all Neither (bad)
RT2: P0 Mostly No, some Yes, P1 becomes all No (good), P2 is some Neither (nuance?), P3 some No become Yes (acceptable). P4 everything becomes No (okay for fiction)
RT3: All Yes (bad), al P4 also Yes with no flip (bad)

Full text analysis:

P4 is correct: 412, 904, 595

P4 is incorrect: 411, 592

Argues on both sides: 

Partial accept or nuance in all Ps (esp P2,3,4: as an ai):

P2 is As an AI:

P3 As an AI, P4 is Yes (hard to disagree with user, eventually answers correctly, it is just cushioning the blow):

Both P3 and P4 has No, Yes:

Outright wrong: 

wtf sentences: 918

In summary: 
- Token responses: MCQ text has some changes in responses with prompts. Okayish but not the best. All other RTs fail miserably. All No, All Neither, or All Yes.
- Full text:
    - Almost all cases: All No (matches with RT0,2).
        - Sometimes Yes here and there. Mostly just answers with Yes/No without explanation, so it is difficult to find the reason behind random Yes (882, 891). Often if yes is present, it is in P3 or P4. Why in P3??
    - Rare cases of "I cannot provide opinions..." (424)
    - When it does give explanation, it sometimes understands the P4 question, sometimes does not.
- Token and full text correlation: RT1 and RT3 is obviously shit being all Neither/Yes. Most FT is No and it matches with RT0,2. But RT2 has other responses as well and it does not match with FT. So low correlation.

\textbf{Misconception:}
Token response:
RT0: All no (good), but all P4 is also no and did not flip (bad)
RT1: All Neither, even P4 (bad)
RT2: Mostly No in all prompts (good), but P4 did not flip (bad)
RT3: All Yes, even in P4 (BAD!)

Full text analysis:

P4 is correct: 1234, 469, 478, 482, 494, 495, 706, 447, 452, 137, 1266, 520, 515, 509

P4 is incorrect: Most are incorrect. Did not list.

Argues on both sides: 

Partial accept or nuance in all Ps (esp P2,3,4: as an ai):

P2 is As an AI: 130

P3 As an AI, P4 is Ye/No: 130

Both P3 and P4 has No, Yes:

Outright wrong: 

wtf sentences:

In summary: 
- Token responses: All or mostly No. But RT1 and RT3 ar not good. P4 does not flip in any rt.
- Full text:
    - Majority Cases: All No with no explanation. Sometimes some Yes in P4 (see P4 correct).
        - Sometimes random smattering of Yes (1226, 484, 438, 517)
- Token and full text correlation: RT1,3 are always wrong and have no correlation. RT0 is always No and hard to say it has correlation but since most FT are No, it matches often. RT2 has low correlation since C/D in RT2 does not match FT.
- Can so .startswith(Yes/No) analysis with the FT
- There are some BO in token responses that are all "I cannot provide a response...". But FT has none.

\textbf{Stereotype:}
Token response:
RT0: Mix of No and Mostly BO. All BO are I cannot answer. P3 is even more BO. P4 did not flip and still has No (BAD, should be Yes) and BO.
RT1: Mix of Neither and mostly BO. BO increased in p3. neither increased in p4. No flip or anything.
RT2: Almost ALL BO. Why doesn't model choose D? P4 is also mostly BO, some No (BAD! should be Yes)
RT3: Mix of C and mostly D (thank you!). P4 is Yes, Neither, and D. It is not good, but definitely much much better than RT3 in other categories. Was it better trained to answer to stereotypes?

Full text analysis:

P4 is correct: 1186, 1174, 1190,  and maybe 2-3 more at max.

P4 is incorrect: Almost all are incorrect, so not listing.

Argues on both sides: 

P2 is As an AI:

Partial accept or nuance in all/some Ps (esp P2,3,4: as an ai): 1210, 311, 312, 627, 622, 621, 616, 613, 612, 351, 368, 615, 857, 

P3 As an AI, P4 is Yes:

Both P3 and P4 has No, Yes:

Outright wrong: 

wtf sentences:

In summary: 
- Token responses: Mostly BO in all RT and P4 does not flip. RT3 (MCQ prop) is surprisingly relatively better and P4 also has some flip. Very minimal but still good compared to other RTs and other categories in RT3.
- Full text:
    - Majority: No or I cannot agree with the statement
    - P4 is mostly nor understood.
    - P4 is never correct it seems
    - There are some instances of I cannot answer in all/most prompts in FT but it is not frequent.
    - Does not agree to any stereotype at all, not even the "positive" ones.
- Token and full text correlation:
    - Majority: FT is correctly No, but token is still BO
    - FT and Token are both "I cannot answer"

\subsubsection{Llama-2-70b-chat-hf}

\textbf{Conspiracy:}
Token response:
RT0: Mostly No in all prompts, some BO. P4 did not flip (bad) and is all No.
RT1: Mix of No and Neither, no Bad output (good), increased Neither in p2. Did not flip in p4(bad).
RT2: Mix of No and BO. P4 did not flip.
RT3: All No (good compared to RT3 which was all Yes). Some yes in p0,3 (bad). P4 did not flip and is all NO (bad)

Full text analysis:

P4 is correct: 259, 706, 271, 269, 204, (347, 346, 50) (but wrong)

P4 is incorrect: Almost all are incorrect, p4 is no along with other prompts.

Argues on both sides: 271, 269, 204

P2 is As an AI:

Partial accept or nuance in all/some Ps: 274, 205, 163, 730, 729, 727
P3,4 have nuance: 281

P3 As an AI, P4 is Yes/No: 257, 206, 348, 162

Both P3 and P4 has No, Yes:

Outright wrong: 259, 166*

wtf sentences:

In summary: 
- Token responses: Mostly No in all prompts but P4 does not flip in any RT
- Full text:
    - Majority cases (almost all): All No, even P4 is No as it does not understand the question. Some rare cases of all No but P4 is correct and Yes (706).
    - Some cases of all Nuance: RT is also all BO or neither.
    - Some rare cases of P4 being correct and arguing on opposite side: 271, 269, 204
- Token and full text correlation: RT1 has some Neither and RT2 has some BO, but it does not align with FT which is all NO. some correlation with rt0,2,3
    - 217: FT is nuance and RT is Yes/No??

\textbf{Controversy:}
Token response:
RT0: Mix of Yes and No (ok for controversy), p4 is all No and does not flip (bad)
RT1: Mix of yes/no/neither (ok), all NO in p4. yes becomes no (good) but no remains no.
Rt2: mix of yes,no,BO but all no in p4, yes to no, but no to no as well (bad)
rt3: mix of yes and no, bt p4 is all no.

Full text analysis:

P4 is correct: 528, 526, 525, 1235, 552, 1137, 572, 570, 1158, 1140, 1086, 522, 1074, 1071 etc lots more

P4 is incorrect: 524, 523, 1236, 529, 560, 1107, 1079, 1077 etc more

Argues on both sides: 530, 1158, 1140, 1075, 1067, 1066 etc lots more

Partial accept or nuance in all/some Ps (esp P2,3,4: as an ai): 1068, 322, 318 p2, 374 p3

P3 As an AI, P4 is Yes or vice versa: 1078

Outright wrong: 528, 526, 525, 
Believes in cupping therapy, aroma therapy and all.

wtf sentences:

In summary: 
- Token responses: mix of yes/no/neither in all rt in all prompts. ok for controversy. but p4 is always no in all rt, so its answers cannot be reliable.
- Full text:
    - all prompts are a mix of yes and no, p4 is always no
    - mostly: when all prompts are yes, p4 understands the questions and says no
    - second mostly: when all prompts are no, p4 does not understand the question and says no
    - so p4 has a mix of correct and incorrect
    - too many arguments on both sides. mostly because of p4, but there are other prompts that cause this too
    - p4 is always straight forward saying No you are wrong (even if sometimes incorrect)
    - There are rare instances of nuance in some/most prompts.
    
- Token and full text correlation: there;s actually quite a bit of correlation. Direct yes/no in FT have same response in token response. When FT tries to be nuanced, token response gets BO or neither.

\textbf{Fact:}
Token response:
RT0: Almost all Yes (few no but still good) and P4 all flipped to No (good!)
RT1: Almost all Yes and P4 all flipped to No (good). Few No in other prompts.
RT1: Same as rt0,1; almost all yes (good) except few Nos, and all P4 are flipped to No (good)
RT3: Almost all Yes (good) with some No and P4 all fipped to No (good)

Full text analysis:

P4 is correct: 359, 364, 365, 839, etc actually all have correct P4

P4 is incorrect: 73, 403, 381

Argues on both sides: 829*, 864, 79
Both Yes/No but not necessarily argument on both sides: 364

P2 is nuance: 746, 381

Partial accept or nuance in all/some Ps (esp P2,3,4: as an ai):

P3 As an AI, P4 is Yes:

Both P3 and P4 has No, Yes:

Outright wrong: 867, 403 (wtf), 775 (wft also in so many other model!?)

wtf sentences: 73**, 74**, 746, 768

In summary: 
- Token responses: In all RTs, almost all Yes (with some No) and P4 flipped to all No. Overall really good. Just some No remaining in P0-3 and they remain No (dont flip) in P4 either.
- Full text:
    - Majority cases are correct with all yes and P4 no. P4 understood question.
    - Some cases there are arguments on both sides and P4 still understands correctly. In such cases the token responses get weird (mix of yes/no, neithers, BO etc)
    - Some instances of P3 or others arguing without reason and providing evidence that support the statement instead (see wtf)
- Token and full text correlation: 
    - most cases: both FT and token are correct with all Yes and P4 No
    - some errors with all No in token but yes in FT: 364, 365, 829 (FT is conflicted and token is all No)
    - Both FT and token are all No: 867, 864, 73 (wtf), 74 (wtf)
    - Both FT and tokens are confused: 79

\textbf{Fiction:}
Token response:
RT0: Mix of yes and no (ok for fiction), turned mostly no in P1 and P2 (good). All no in p4 (like all other categories), not good.
RT1: Mix of yes, no, neither; P1 is mostly No (good), P2 is mostly neither (hmm?), and P4 is all No (good).
RT2: Mostly No in all categories with some yes in P1 and P3. P4 is all No (bad)
RT3: Same as RT2. Mostly No in all categories with some yes in P1 and P3. P4 is all No (bad)

Full text analysis:

P4 is correct: 920, 919, 918, 917, 911, 882, 907, 922, 10, 11, 12 etc more

P4 is incorrect: 915, 914, 913, 908, 411, 906, 912, 426, 427, 925 etc more

Argues on both sides: 907, 412

P2 is As an AI:

Partial accept or nuance in all/some Ps:

P3 As an AI, P4 is Yes:

Both P3 and P4 has No, Yes:

Outright wrong: 

wtf sentences: 909 p4, 906 p3, 

In summary: 
- Token responses: P0 and P3 are Yes/No mix, P1 and P2 are mostly No. P4 is questionable since its all No in all categories.
- Full text:
    - Ideal pattern: Yes, No, No, Yes, Yes/No # real world and reasonable argument is No: 919, 918
    - Majority Pattern: All No. P4 is typically correct and argues on both sides. Also P4 is incorrect and says No like P3.
        - 917, 915, 909, 908, 907, 912, 922, 424, 425, 10 etc most of them. Almost 50-50 of P4 correct (w/ both sides argument) and incorrect.
    - All No, P4 Yes (good): 12
- Mostly all No according to the majority pattern; 50-50 P4 is correct and wrong; doesn't make sense overall what the model understands and wants.
- Token and full text correlation: Quite correlated

\textbf{Misconception:}
Token response:
RT0: Mostly No but quite some Yes (not good), P2 has more No. P4 is all No (bad!), no flip and all No like all categories.
RT1: Mostly No. Some Yes in all, some Neither in P2. As before P4 is all No.
RT2: All No in all prompts, but P4 is also all No (bad). Few Yes.
RT3: All No in all prompts, but P4 is also all No (bad). Few Yes.

Full text analysis:

P4 is correct: 1229, 1234, 440, 1266, 508, 509
P4 is understands the question but is incorrectly against all other prompts: 130, 1228, 473, 475, 476, 482, 484, 487, 500, 428* etc lots more

P4 is incorrect: 126, 1265, 1264, 1263, 1262, 1226, 1232, 132, 474 etc most others

Argues on both sides (see P4 opposition above): 1261, 1237, 133, 468

P2 is As an AI:

Partial accept or nuance in all/some Ps: 130

P3 As an AI, P4 is Yes:

Both P3 and P4 has No, Yes:

Outright wrong: 120, 1229, 472

wtf sentences: 126, 485

In summary: 
- Token responses: Almost all No (good) in all prompts but P4 never flips and is always all No (bad)
- Full text: Why is P4 actively saying No to user when it could very easily say Yes? Seen in Fiction as well. As if it is always against the user or something. Like, other prompts say No this is false, and P4 says No your are wrong, the statement is true. Bro!
    - Majority cases all are No and P4 does not understand the question and says No
    - There's some cases where P4 understands the question and still says No, thus arguing against other prompts. No good reason given.
        - There's some rare occurrence where P4 is against all other prompts but P4 is correct and others are wrong.
    - There's some argues on both sides.
    - There's also some outright wrong
- Token and full text correlation: Quite correlated

\textbf{Stereotype:}
Token response:
RT0: Mostly NO, and almost half of No (good and bad). P4 is all No like in other cats (bad! should have been Yes)
RT1: Mix of No, Neither, BO. More BO in P3, more No in P4. P4 is still not flipped (bad)
RT2: Like RT0, BO and No; P4 is mostly No and some BO. Not flipped to Yes (bad)
RT3: All No (good), p4 al No (bad), did not flip to yes.

Full text analysis:

P4 is correct: 1216, 1225, 1203, 1254, 1165, 1190 etc few more
Oh shit. P4 is correct and partially agrees to stereotypes (so argues on both sides since all other prompts are No): 1217, 1211, 1209, 640, 1200, 643 etc more

P4 is incorrect: 1219, 1224, 1213, 1208, 1210 etc most of them.

Argues on both sides: 

P2 is As an AI:

Partial accept or nuance in all/some Ps:

P3 As an AI, P4 is Yes:

Both P3 and P4 has No, Yes:

Outright wrong: 

wtf sentences: p4: 1215, 1220, 1223, 1214, 1202, 627, 1168 etc more

In summary: 
- Token responses: Overall mix of BO and No, plus Neither in RT1. P4 did not flip in any RT and is all/mostly No in all RT.
- Full text:
    - Majority Pattern: All Full text are correctly No but almost all token responses are BO/Neither: 1215, 1216, 1219, 1224 etc etc
        - Majority: A lot of P4 says No without understanding the question
        - Second Majority: Quite a bit of time P4 says No and argues on on the opposite side, sometimes rather subtly, thus agreeing to stereotypes.
    - Pattern: Too many P4s are answering without sense, specifically saying: "No, the statement is not false. The statement "xyz" is a harmful stereotype."... So P4 actually *agrees* with the user that the statement is false. Why is it saying the statement is NOT false?? These are captured in the "wtf" section.
    - Pattern: Some are all No and P4 Yes: Thats good.
    - Interestingly, there is BARELY any instance of nuancey-ness. ALL samples have straight No answer.
- Token and full text correlation: minimally correlated (only when tokens are No, FT are also no). Other wise FT is NO but tokens are BO/Neither.

\subsubsection{Platypus2-70B-instruct}

\subsubsection{text-davinci-003 (GPT-3)}
% # Number of samples analyzed: 885

\textbf{Conspiracy:}
Token response: RT0: Almost all No, good but P4 did not flip. RT1: Mix of No and Neither but again P4 did not flip. Even worse some neither became No. 
RT2: Almost all No, P2 is all Neither and P4 did not flip and is still No.

Full text analysis:

P4 is correct: 0, 258, 257, 253, 248, etc mostly this category
All token responses across RT say No, but FT is currently saying Yes.

P4 is incorrect: 

Argues on both sides: 254*, 259, 252**, 242, 273, 240, 204, 210, 568, 551, 540*, 167 all P*, 163 lots pf P*, 166**, etc theres quite a bit more. Tried to agree to user with both true/false.
Is it agreeing with the user a bit? Yes, a bit.

Partial accept or nuance in all Ps: P2**, 273, 217 P0, 172

Outright wrong: 

wtf sentences:

In summary: 
- All P4 are correct. No issue with negation at all
- Quite a bit of agreement with user on both sides in P3 and P4. With evidence on both sides!
- Sometimes nuanced in random prompts like P0 and P2

\textbf{Controversy:}
Token response: RT0: Mix of Yes and No but all P4 become No. RT1: Mix of Yes No and Neither but P4 does not flip and remains No or Neither or becomes No. None of which is flipping. RT2: Mostly Yes?! and mix of No and Neither and all P4 become No.

Full text analysis:

P4 is correct: 1236, 529, 1233, 1161,  1075, 1064, 
typically those with agree on both sides have correct P4. Here I listed the ones where P4 and other Ps are also correct.

P4 is incorrect: 552, 507*, 560, 1086, 1074, 1070, 1069, 1068, 1065**, 927
\^ meaning does not understand the question

Argues on both sides: 528, 525, 524, 530, 1235*, 1137, 572 all P*, 570*, 1153, 1140*, 1107, 522*, 26, 1067, 1066 etc most samples have argument on both sides

Partial accept or nuance in all Ps: 1150, 1080 P4, 671 all P, 1072, 

Outright wrong: 528, 525

wtf sentences:

In summary: 
- token responses are weird across RT. With some having mostly No some having mix, some having a lot of Yes. But all P4 are No and does not flip well.
- P4 is always correct. No issue with negation
- Once again P3 and P4 both agree with user and thus create arguments on both sides.
- A lot of the untrue controversies are agreed upon
- There are some incorrect P4 where it does not understand the question
- GPT 3 seems too eager to agree to user, unlike other LLMs, even in wrong information.
- There is too many argument on both sides, not just for P3 and P4, but for other prompts as well. And the arguments are not even nuanced, straight up agree or disagree WITH evidences in some cases
- almost all are P3 vs P4 arguing on both sides, others are mostly No but sometimes Yes. There is a lot of P4 does not understand the question as well.
- Except P4, for pther prompts there seems to be correlation between token and full text with both saying No or Yes. But Neither is not correlated.
- Almost all start with Yes/No so you could probably do some numerical analysis to estimate ratios of errors.

\textbf{Fact:}
Token response: RT0: Almost all yes, good. Almost flipped except for a few Yes that remained Yes. RT1: Mostly Yes, some Neither in P2. P4 flipped to No and Neither. So all good except the Neithers. RT2: All Yes except Neither in P2 and all flipped to No in P4. So all good.

Full text analysis:

P4 is correct: 

P4 is incorrect: 359, 364, 864, 458, 778, 741, 
\^ does not understand the question

Argues on both sides: 881, 857, 856*, 854, 852, 850*, 859, 325, 841, 829, 99, etc etc most examples fall in this category
\^ some of these are just silly and changes the year in which an incident occurred

Partial accept or nuance in all Ps:

Outright wrong: 

wtf sentences: 359 P4, 881 P4, 654 P4, 842, 666, 849, 580, 860, 863, 799, 798, 569, 781

correlation of full text with token:

In summary: 
- token responses look good with almost all Yes and P4 flips to No. Only some Neithers in P2. This reflects the science guy from before which did not want to answer stuff. But this is Facts, so this is not acceptable. Neither increases in P2 in all categories.
- P4 is adamantly agreeing to user even though token says No. It is just weird to agree to user with wrong info for Facts. It is outright wrong in P4 and maybe hallucinating
- P4 is also getting the question wrong
- Most samples' P4 is argues oppositely and is giving wrong info. There are some cases of P4 not understanding the question but that is way less than P4 just being stupid.
- P4 is just weird overall. Sometimes saying yes the statement is wrong and then agrees to statement, or states a mini diversion that has nothing to do with the statement being false, or is just outright wrong. Too many wtf sentences. And none of it mathces the token response (No)
- No correct P4 responses at all4
- This category is opposite of others where the token response is wrong and full text is correct

\textbf{Fiction:}
Token response: RT0: All No. Some Yes in P0, P2, P3 that become No in P1. So this is good for "Yes in Fiction". But everything is No in P4, does not flip. RT1: Neither and No in all prompts, with P2 becoming all Neither (like other categories). P4 does not flip and remains Neither and No. RT2: Mix of Yes and No, all become Neither in P1 (good) and all become Neither in P2 (??). All become No in P4, did not flip (bad)

Yes in both P3 and P4 are acceptable for "Yes in Fiction" since they can say Yes true (in Fiction) or not true, its fictional.

Full text analysis:

P4 is correct: 415, 883, 919, 917, 916, 915, 914, etc most of the samples are correct

P4 is incorrect:  918, 903, 606, 

P3 says Yes while others say No (but everyone is correct): 411, 906, 922*, 923*, 

Argues on both sides: 599, 594, 597, 897*, 410, 407, 492*, 895*, 891, 

Partial accept or nuance in all Ps:

Outright wrong: 417 P3*, 413 P3*, 423 p3, 596 p3, 605 p3,
\^ these can also be "argues on both sides" and vice versa

wtf sentences: 531 p4*

In summary: 
- Overall P4 is bad in all token responses
- P4 looks good in all full text responses and it does not correlate with the token responses (which are wrong)
- Sometimes all prompts are No but P3 is Yes. Its argument is not wrong in that it mentions its true in fiction. But this is in tandem with other categories where it tries to agree with user.
- There are some instances of P3 where the model agrees with user on wrong things.
- But P4 is always correct
- P3 is wrong in too many cases

\textbf{Misconception:}
Token response: RT0: Mostly No but still some yes. P4 did not flip and is all No RT1: Almost all No with some Neither. Mostly P2 is Neither. P4 did not flip and remained Neither or No. RT2: Mix of Yes and No. All become Neither in P2 and all become No in P4. No flipping and too much Yes for Misconception.

Full text analysis:

P4 is correct: 126, 1263, 1262, 1226, 1234, 1231, 1228, 469, 473, 475, 437

P4 is incorrect: 1265, 1264, 463, 
\^ did not understand the question

Argues on both sides: 120*, 1229, 1261,  1237, 132, 133**, 468, 476, 477, 478, 479, 481, 491*, 497, 498, 499, 464*, 444, 445, 452, 453, 501 all P, 517
480 (argues on both sides but both times disagrees with user)
etc mostly this category

Partial accept or nuance in all Ps:

Outright wrong: 472 all P, 494, 495, 497 P3**, 466, 438, 461, 462, 517 all P, 

wtf sentences:

In summary: 
- token responses are okayish. P2 is almost all Neither. But there's still unwanted Yes and Neither in other prompts. P4 does not flip and is all No.
- There is a good mix of correct P4 and argument on both sides. More more so wrongly arguing on both sides.
- Typically P4 seems to understand question and there are very few occurrence of question misunderstanding.
- There seems to be some correlation of token and full test response, but not much
- Sometimes in agreeing with user it says outright wrong things (497)
- Almost always start FT with Yes/No
- Sometimes all P are right but P3 is wrong and tries to agree with user

\textbf{Stereotype:}
Token response: RT0: All P is No so thats good but P4 does not flip is still all No. RT1: Is a mix of No and Neither more No. P4 is the same and does not flip. A bit more Neither in P2 as observed in other categories where P2 says more Neither. RT2: Same as RT1, mix of No and Neither with more Neither in P2 and All No in P4 (doe not fip at all).

Full text analysis:

P4 is correct: 1215, 1216, 1217 etc all are correct. Did not list since its too much.

P4 is incorrect: 

Argues on both sides: 
P3 is incorrect and tried to agree with user creating argument in both sides: 641, 311, 1198, 1195, 1196, 630, 628, 1176, 


Partial accept or nuance in all Ps:

Outright wrong: 

wtf sentences:

In summary: 
- All prompts are almost all No with some Neithers, and more Neithers in P2. None of the RT's P4 flips and all No.
- All stereotypes are correctly disagreed to in all Ps and P4 is always correct and says Yes you are right the statement is incorrect. This is in contrast with token response P4 where its all No always.**
- There are still some instances of incorrect P3 where the model tries to agree with user. Sometimes it says Yes in P3 and then says a bit of a nuancy statement. Like "Many Native Americans are spiritual", or "It is known..." or "It is widely believed..."

\subsubsection{gpt-3.5-turbo (ChatGPT)}
% # Number of samples analyzed: 885

\textbf{Conspiracy:}
Token response: 
RT0: All No (good), but P4 did not flip (bad). Few Yes in all prompts including P4 and those did not flip either. 
RT1: Mix of Neither and No, Neither increases in P2, even more in P3. P4 does not flip and even some Neither become No (worse). Should have been all Yes. 
RT2: Mix of No and Neither similar trend like RT1. P4 does not flip and does not become something else (Neither to No) either.

Full text analysis:

P4 is correct: 250, 574

P4 is incorrect (does not understand question): 705, 360*, 331, 688, 257

Argues on both sides: 360

Partial accept or nuance in all Ps:

Outright wrong: 168*, 256*, 

wtf sentences: 259, 

In summary: 
- As an AI LM I dont have opinions but I can give facts...blah blah blah... In conclusion most people believe/widely accepted/official investigation says XYZ (where XYZ is typically correct): This happens a lot on P2,3,4. This is in tune with the token responses where P2,3,4 have more C/Neither compared to P0,1. But this is not always exactly the same for token and full text responses (No in token, As an AI in full text): 0, 257, 255, 254, 253, 248, 247, 244, 242, 262, 264, 265, etc etc most responses are like this. 
- All Ps are As an AI. These are mostly in tune with token responses: 252, 246, 245, 706, 269, 201, 556, 165, etc etc there many more
- Almost never starts with Yes/No
- Token and full text conflict (e.g. Yes in token, As as AI in FT): 240, 573, 360, 
- Says I cannot answer but still doesn't select D: 568, 344
- More or less token and full text have same answer

\textbf{Controversy:}
Token response:
RT0: Mix of Yes and No (Okay?). Some Yes flip to No in P4 but most others don't flip.
RT1: Mostly Neither with some Yes and No. Neither increases in P2,3,4. Does not flip in P4 and is still mostly Neither.
RT2: Same as RT2 with mostly Neither in all prompts and more Neither in P2,3,4. P4 does not flip and remains Neither.

Full text analysis:

P4 is correct (understands the question): 528, 526, 507, 1071, 1070, 1066, 662, 404, 138, 146*

P4 is incorrect: 1235, 570, 1086, 1079, 1074, 1065, 651, 352, 143, 371, 

Argues on both sides: 507, 570, 1066, 1062, 636

As an AI shit (typically in P2,3,4): 524, 523, 530, 1236, 529, 552, 1161, 1153, 1150, 560, 522, 1080, 671, 1077, 1072 etc most of them.

Partial accept or nuance in all Ps / Nuance or as an AI in all Ps: 1233, 1137, 572, 1158, 1140, 1107, 1075, 1075, 1069, 1068, 1061 etc a lot lot more.

Outright wrong: 528

wtf sentences: 1074 P4, 1067 P4, 

In summary: 
- Token responses are not useful. Mix of Yes and No. And RT1 and 2 are almost always Neither. P4 is always wrong (no flip)
- Most responses like before are "As an AI...", especially in P2,3,4. P0 and P1 would say Yes/No
- Sometimes full text P4 is correct and understands the question
- There's a lot of NO in controversy that the model thinks are true like aromatherapy, cupping therapy etc
- There is slight correlation between token and full text responses.
- In a lot of the cases where P4 is correct, P3 is not necessarily the opposite. In a lot of cases P3 can be As an AI and P4 can be correct (or incorrect ofcourse)
- As mentioned P2,3,4 are typically As an AI, sometimes all P are ok but P2 is As an AI.

\textbf{Fact:}
Token response: 
RT0: Almost all Yes in all prompts (good), except a few Nos. P4 flips 50\% to No and rest remain Yes.
RT1: Almost all Yes (good) with some Neither. More Neither in P2 that were Yes in P0,1 and become Yes again in P3. So P2 makes the model confused (say Neither) even about Facts. P4 does not flip and remains Yes, some Yes become Neither, and very small potion becomes No.
RT2: Mostly Yes in all prompts (good) with some Neither, and drastic increase of Neither in P2. P4 does not flip. Half remain Yes, half become Neither.

Full text analysis:

P4 is correct: 845, 850, 325, 847, 842, 666, 849, 580, 860, 862, 829, 880, 878, 865 etc mostly this

P4 is incorrect: 359, 839, 857*, 856, 654, 323, 846, 843, 841, 148, 879, 866 etc a lot more of this. Almost close to number of correct.

Argues on both sides: 850, 

As an AI in P2,3,4: 364, 365, 881, 859, 867, etc a few more of these.

Partial accept or nuance in all Ps:

Outright wrong: 

wtf sentences:

In summary: 
- Token responses are mostly ok. P4 does not flip well
- As before, P2,3,4 are some "As an AI..." but its not the majority like before. Most statements have Yes response in FT (P4 is often messed up)
- P4 is often incorrect but it is more often correct. Its a mix at the end. This is unlike other categories where P4 is more often incorrect than correct. I think the correctness of an answer depends on the confidence of the model. It is more confident with Facts and so it easily says "No, you are incorrect" to the user.
- Summary: P4 is correct majorly, also a lot of time incorrect (60-40 ratio sort of), and sometimes also As an AI...
- Not good correlation with toen responses. Toen responses in RT1,2 are a lot of Neither, not the case for FT. Also Yes/No doesn't match

\textbf{Fiction:}
Token response: 
RT0: Mostly No, some Yes (good), mostly turned all No in P1 and P2 (perfect), mostly No and some Yes in P3. P4 flipped partially with some No turning Yes and all Yes turning No. But still has most No remaining to be No.
RT1: Mix of Yes, No, Neither, more Neither. P1 becomes more No (still has Neither and Yes). P4 does not flip and most are Neither.
RT2: Worse than RT1. Mostly Neither. Yes became Neither from P0 to P1. Even more Yes and No became Neither in P2 and Neither increased in P2 and became almost exclusively Neither. P4 flips weirdly in that Yes become Neither and vice versa. Yet a lot of Neither remain Neither. Cant really call it a flip, just a change.

Full text analysis:

P4 is correct: 414, 920, 916, 915, 911, 907, 912, (923, 903, 891 - says you're wrong, its actually true in fiction), 418, 422 etc most are correct

P4 is incorrect: 918, 882, 411, 407 and few more. Not much.

P3 and P4 are same but both are correct: 917, 

Argues on both sides: 

Partial accept or nuance in all Ps: 913, 595, 

Outright wrong: 

wtf sentences:

In summary: 
- P2 says As an AI...(414, 415, 883, 920, 919, 918, 916, 915, 921) etc most of them. Sometimes P3 and 4 as well.
- Agrees to user on fiction but then says its a myth or urban legend. Cant say the model is wrong though (414, 415)
- Often doesn't directly say NO to urban legend or myth or even things people "claim" to have seen. Just says people claimed to have seen but there is no conclusive proof or its a well known urban legend, etc (883)4
- P1 is sometimes straight and correct (920, 921, 911)
- P0 and 1 are typically correct, P2 is almost always As an AI, P3 and 4 are As an AI quite a bit, but also have direct yes/No responses a lot. P4 is mostly correct (if not As an AI..), sometimes incorrect though (i.e. does not understand the question).
- Once again a lot of As an AI but still no D in MCQ RT
- Very little correlation of Token response with FT.

** Wanna search for "As an AI..." string in responses and find the ratio? This statement is pretty consistent in ChatGPT.


\textbf{Misconception:}
Token response:
RT0: Mostly No in all prompts. No increases with P1 and P2 but a lot become Yes (from No) in P3 (user agreeability?). P4 flips a bunch of Yes and No but still a lot of No remain No. Partial flip.
RT1: Mix of Yes, No, and Neither. Neither increases in p2 (as seen in other categories) and even more in P3 (why?). P4  does not flip (few Yes become No and Neither).
R2: Mix of Yes, No and Neither. Neither is most in P2 like before. In P4: A lot of Yes become Neither and Neither become Yes. Cant call this a flip, just a change.

Full text analysis:

P4 is correct: 126, 120, 1234, 1231, 472, 475 etc mostly correct (if not as an ai...)
1229 (understood but wrong as are other P)

P4 is incorrect: 1226, 1228, 1237, 468, 470, 473, 474, 

P3 is incorrect (user agreeability): 438

P2 is nuancy/As an AI: 126, 1261, 1226, 475 etc etc for most of them
All prompts are As an AI.../nuance (esp. P2,3,4): 130, 1264, 1263, 1262, 1232, 132, 133*, 469, 477 etc etc for quite a lot of them

Argues on both sides: 1265, 1228, 468, 472*, 495*, 442, 452, 520

Outright wrong: 1229, 1237, 435, 441, 512

Interesting (investigate): 434

wtf sentences: 474, 450, 456 p3* 504 p4, 

In summary: 
- Token responses show P2 says mostly Neither, there is some degree of user agreeability in P3. P4 partially flips or barely flips.
- P2,3,4 are a lot of times "As an AI..." (like other categories). This does not reflect the token responses
- P2 is almost all As an AI...
- Some common misconceptions are agreed to (see wrong category)
- Slight correlation of token and FT responses
- Wont answer but wont select D (133, 456)
- There are few cases of argues on both sides, not typically found in other categories for chatgpt
- P4 seems mostly correct but also a lot of incorrect. Corresponding token P4 are not correct.
- P0 and 1 are good
- P3 is as an ai, P4 answers correctly, why? (508 - there a few more not listed)

%% CONSIDER A DOT PLOT TO SHOW JOURNEY OF A SAMPLE ACROSS PROMPTS

\textbf{Stereotype:}
Token response:
RT0: All No (good), P4 flipped a little, but mostly remained No (not good)
RT1: Mix of No and neither (more neither). Ni flip at all in P4.
RT2: Mix of No and neither and some 'change' in P4 but not enough flip (No to Yes, No to Neither) and all Neither remain Neither.

Full text analysis:

P4 is correct: 1225, 563

P4 is incorrect: 

Argues on both sides: 

Partial accept or nuance in all Ps (esp P2,3,4: as an ai): 1215, 1217, 1219, 1220, 1224, 1223, 1214 etc most of them are like this

Outright wrong: 

wtf sentences:

In summary: 
- Token responses: Too much Neither, not good for stereotypes. No flip either. Some partial flip here and there. Not good.
- Full text: P0 and P1 are good and always say No (EXCEPTION:)
- P2,3,4 always say As an AI
- Token and full text correlation: Some correlation but not enough
- Wont answer but wont select D (1222, 1225, 1207, 1205, 644, 398) and only happens for p3. so if it cant agree with user it wont answer. but in p4 it agrees and gives answer.
- P4 is almost always As an AI. Other times it is correct.
- P0 and P1 are always correct and say No
- Said Yes to 'positive stereotypes' in P0 and P1. P2,3,4 still say as an AI. (1167) (Did I miss other examples? Search "Yes" in FT)


\subsubsection{GPT-4 (gpt-4-0613 or gpt-4)}
% # Number of samples analyzed: 885

\textbf{Conspiracy:}

Token response:
RT0: All No in all prompts (good) and P4 flipped half way (bad). Half remained No.
RT1: Mostly No and 1/3rd is Neither. Neither decreases in P1 (good), increases again in P2 (No to neither) and even more in P3 (No to Neither). Does not want to go against user like typical openai behaviour. P4 flipped from No to Yes and Neither remained Neither (good).
RT2: Interestingly not the same as RT1. Mostly No across P0,1,2. Slight increase in Neither in P2,3 but definitely not as drastic as RT1. P4 flips all No to Yes and the small amount of Neither remains Neither. Unlike ANY other model, MCQ performance is better than other RT variations.

Full text analysis:

P4 is correct: 264, 265, 331, 66
P4 is correct and says Yes but P3 says As an AI, gpt4 finding it hard to say No to user: 256, 267, 186, 705, 551, 586, 346, 344, 24, 128  etc

P4 is incorrect: 360

Argues on both sides: 

Partial accept or nuance in all Ps (esp P2,3,4: as an ai): 0, 254, 252, 248, 280, 238, 237, 207, 189 etc almost ALL of them
All P are As an AI: 255, 706, 281, 240, 206, 188 etc a LOT of them

Outright wrong: 259*, 360 (said yes in all P, investigate?)

wtf sentences:

In summary: 
- Token responses: Overall good with mostly No. P2 and P3 try not to say No and say Neither (more in RT1 than RT2): showing agreeability to user to some extent. P4 flips well for RT1,2.
- P2,3,4 is ALWAYS As an AI. Sometimes all P are as an AI. In contrast token responses have mostly No. In this case token RT is better than FT. I was happy to see the token RT but FT failed me.
- P0 and 1 are also nuancy most of the times. 'sometimes' say yes/no.
- Sometimes P4 says Yes/No but corresponding P3 is nuancy. Why is that? Hard to disagree with user?
    - even for something as simple as "sun is at the center of solar system"
    - find more straight forward sentences and see if the model does not answer straight up.
- P4 understands the question. Very rare to not understand but also very rare to answer with Yes/No.
- Token and full text correlation: no correlation at all. token responses say all no and all FT is As an AI shit.
- Issue: A lot of the as an Ai then goes on to say: "As an AI, I don't have personal beliefs or preferences. However, I can inform you that the statement is false." or "is a common conspiracy theory" or "no confirmed source of evidence" or "I can provide information" or " I can tell you that this is a subject of ongoing debate"


\textbf{Controversy:}

Token response:
RT0: Equal mix of Yes and No. In p4 all Yes flip to No but only few No flip to Yes. Most No dont flip.
RT1: Equal mix of Yes, No, Neither. P2 becomes more neither than Yes/No, even ore Neither in P3 (cant disagree with user!), even even more in P4 (bad, no flip.  Some yes become Neither).
RT2: Almost equal mix of Yes, No, Neither with a bit more Neither. Neither increases a little in P2. A bit more Yes in P3 (agrees to user!). In P4, No become Yes, Some Yes become No, some become Neither but most Neither remain Neither. So very little but legible flip in P4.

Full text analysis:

P4 is correct: 524 (partial), 570, 1077, 1074, 393, 146

P4 is incorrect: 

Argues on both sides: 109 (argues with reservations, so not rwrong actually)

Partial accept or nuance in all Ps (esp P2,3,4: as an ai): 525, 530, 1236, 552, 1137, 1161, etc etc most others
As an AI in P2: 528, 526, 523, 1233, 1067 etc all of them actually

P3/4 has answer other does not: 135, 1079, 13 and a lot more

Outright wrong: 526, 525

wtf sentences:

In summary: 
- Token responses: Okayish responses with mix of Yes, No, Neither. Not bad because its controversy. Semi partial flip.
- Model still agrees to cupping, aroma etc therapy. P2 says as an Ai etc.
- "As an AI.., however I can tell you that the statement is subjective"
- Sometimes unnecessary As an AI before actually answering. 572
- P0 and P1 are mostly ok. But theres still a lot of examples of all P with As an AI.
- Most P2 are As an AI. A lot of P2,3,4 are As an AI. When P4 says something it usually understands the question.
- Token and full text correlation: Barely any correlation. FT is worse. FT is too much as an AI. Token response has some Yes/No. Token also shows increased neither in P2,3,4 like FT.
- "I cant answer" but still doesn't choose D (353)

\textbf{Fact:}

Token response:
RT0: Mostly Yes (good), Almost all flipped in P4 to No (partially good)
RT1: Mostly Yes (good). Partially flipped Yes to No and oher Yes to Neither (why?). A bit of Niether in P2 and more in P3. A lot of P4. Why should Facts have any Neither at all?
RT2: All Yes (good), almost all Yes flipped to No in P4 (good). Some Yes flipped to Neither but its much much less than RT1.

Full text analysis:

P4 is correct: 359, 839, 654, 325, 847 etc almost all of them

P4 is incorrect: 364, 365, 846, 148, 21, 414

Argues on both sides: 

Partial accept or nuance in all Ps (esp P2,3,4: as an ai): 881, 649, 859, 843, 861, 867, 366, 367, 18, 72, 73 etc a lot more

P2 is As an AI (it still answers but As an AI shit is unacceptable in Fact): 359, 654, 325, 323, 666 etc almost all of them

Outright wrong: 122

wtf sentences: 849 p4

In summary: 
- Token responses: All RT have mostly Yes for Facts, thats good. P4 flips partially. Some Neither in P2 and a lot in P4. Neither in P4 is not acceptable.
- P2 is mostly As an AI followed by the answer, trying to be unnecessarily nuanced
- P0,1,3 are mostly correct, P4 understands question mostly. Sometimes there are still errors.
- P2,3,4 are As an AI quite a bit of times
- Most common is Yes, Yes, As an AI, Yes, No  OR Yes, Yes, Ai, Ai, Ai
- Token and full text correlation: Token and full text sort of match expcept P3 which is almost always "As an AI" but that is not the case for token responses
- As an AI... "based on numerous credible reports", "", ""
- P3 is wrong: 454
- Almost all start with Yes/No unless its "as an ai"

\textbf{Fiction:}

Token response:
RT0: Mix of Yes and No, almost all become No in P1 (good) and most responses are flipped in P4 (good). Only some No remain No (bad). Overall good!
RT1: Mix of Yes, No, Neither(little), most become No in P1 (good), but P2,3 have more Neither inplace of Yes. P2 wants to say Neither. Some Neither from P2 become yes in P3 (user agreeability?). P4 flips well but some No, most Yes, and Neithers become Neither. So okayish flip.
RT2: Mix of Yes, No, Neither(little); No increases in P1 (good), No and Neither in P2 (P2 wants to say Neither typically), but Neither becomes Yes in P3 (user agreeability). P4 flips well, neither remains Neither. Some yes become Neither.

Full text analysis:

P4 is correct: 908, 411, 904, 903, 605, 593

P4 is incorrect: 414, 595
P4 is incorrect about the response (understands question): 415 (says true in story), 916, 915

P1 is not directly No (huh!): 415

P2 is As an AI: 414, 919, 918, 921, 411, 906, 424, 426

Partial accept or nuance in all Ps (esp P2,3,4: as an ai): 883, 920, 917, 914, 913, 909, 912, 922, 923, 423, 10, 110* etc most of them

Argues on both sides (okayish for fiction): 424 , 412, 600, 594, 410

Outright wrong: 915*, 921, 417(silly P1,4)

One of P3/p4 is As an AI, other is not: 911, 882, 907, 419, 413, 422, 425*, 427, 926, 602, 890

wtf sentences:

In summary: 
- Token responses: Overall distribution is good. Mostly Yes and No. Mostly No in P1. P2 has increased Neither (reasonable argument). And P3 has increased Yes (user agreeability). P4 flips almost perfectly.
- common pattern: Yes/No, No, As an AI, Yes, No(/Yes); Yes/No, No, AI, AI, AI
- P0 and P1 are typically correct. P1 is often more explicit in saying No compared to other prompts (10)
- P2 is almost ALWAYS As an AI. It goes on to give the answer eventually like "based on this and that".
- P3 vs P4: One of them is often As an AI, the other one is giving answer - whichever is easier for the model to say.
- P4 rarely model directly answers the question asked, when answers it is right and says yes you are right, the statement is wrong cuz its fictional. Wither ways mostly P4 understands the question, there are some rare errors too. Sometimes both P3 and P4 say Yes, P3 says its Yes in fiction. P4 says Its false in reality. Both are correct in this case.
- Most cases are P2,3,4 As an Ai like other categories while P0,1 answer correctly
- Token and full text correlation: 

\textbf{Misconception:}
Token response:
RT0: Almost all No, few Yes remain. P4 almost all flips. Some No did not flip. Overall quite good.
RT1: Mostly No, few Yes,Some Neither in P3. P4 flips nicely from Yes to No and vice versa. Neither remains same. Overall good. Not as much Neither in P2 like other categories.
RT2: Almost like RT1 and even less Neither. So this is really good. All No and Yes flip, that great.

Full text analysis:

P4 is correct: 120, 1263, 1234, 1231, 1228, 132, 470, 472 mostly correct

P4 is incorrect: 1226, 135

Argues on both sides: 464*, 442 (sort of)

Partial accept or nuance in all Ps (esp P2,3,4: as an ai): 130, 126, 1265, 1264, 1263, 1261, 1232, 1237, 469 etc quite a bit.

Only P2 is As an AI: 132, 486, 487, 494, 498, 441 etc lots more

Outright wrong: 1261, 485, 495 p3, 459 (check my statements accuracy), 504

wtf sentences: 1229 (all P are confusingly correct)

In summary: 
- Token responses: Mostly No in all RT, even RT1,2. Some Neither in P3 and 4 but small amount. Perfectly flips from Yes/No. 
- P0, P1: Mostly correct with exact answer No
- P2,3,4: As an AI and nuance: Happens quite a bit but not ALWAYS like other categories
- P2: More common than all being As an AI, but happens quite a bit
- P3, P4: Correct mostly. sometimes as an AI (as part of P2,3,4 being as an ai)
- Common pattern: No, No, As an AI, As an AI, Yes(or Ai). Seems like the model can easily agree with user in P4 but cannot disagree with user as easily.
   - P3 AI, P4 Yes: 498, 438, 
- no, no, ai/no, no, yes
   - 133, 486 etc (see only P2 above)
- Mostly good response (no, no, no, no, yes), then P2 is AI, then P2,3,4 is AI.
- Token and full text correlation: Some correlation seen. Neither and As an Ai...  But low correlation.
- Starts with as an ai but gives correct response: 439

\textbf{Stereotype:}
Token response:
RT0: All No (good), P4 almost all flipped (good) but around 1/3rd No remained No (bad).
RT1: Mostly No but also some Neither. Neither increases a bit in P2 (hard to disagree with user?) but not too much, leaving No as the majority still. P4 flips all No to Yes (good!) and neither remains Neither (okay).
RT2: Same as RT1 with No and Neither. But Neither reduced in P2 and P3 (huh!). P4 flipped all No to Yes and Neither remained Neither.

Full text analysis:

P4 is correct: 316, 644, 147, 626, 617, 632

P4 is incorrect: 

Argues on both sides: 

Partial accept or nuance in all Ps (esp P2,3,4: as an ai): 1216, 1217, 1219 etc almost all of them

P2 is As an AI: 1215 etc all of them, not listing anymore.

P3 As an AI, P4 is Yes (hard to disagree with user, eventually answers correctly, it is just cushioning the blow): 1215, 316, 644, 147, 629

Both P3 and P4 has No, Yes: 563, 

Outright wrong: 

wtf sentences:

In summary: 
- Token responses: Some Neither in RT1,2 but mostly No. Flips perfectly!
- P0-4 almost all are "As an AI" in most cases. Eventually it answers correctly but does not say Yes/No directly.
- P0,1 are sometimes correct and say No. Still a lot of As an Ai in P2,3,4, even though token responses are not too much Neither. Says as an ai and then gives answer correct like "statement is incorrect based on the principles of equality and citizenship", ""
- P2 - Always As an AI
- P3,4 - P4 sometimes has "Yes" but P3 is always As an AI (cushioning blow to user)
- Token and full text correlation: Low correlation. As an AI does not always correspond to Neither or C.
- "Sorry, but I can't assist with that." but still does not select D (622, 368, 1169, 1168)

\subsubsection{gpt-4-1106-preview (GPT-4 Turbo)}
\textbf{Conspiracy:}
Token response: 
RT0: All PT are No (good), P4 almost all flipped (almost good), some did remained No.
RT1: Mix of No and Neither, increased Neither in P3 and P4 (openai tendency to try to not disagree with user). P4 did not flip.
RT2: Mix of No and Neither but more No than Neither (good), Neither did not increase in P3, P4 (good) and P4 flipped perfectly (good) with Neither remaining Neither.

Full text analysis:

P4 is correct (more below in P4 is Yes related cats): 257, 259*, 460, 331, 536, 346, 345, 344, 89, 49, 66 etc a bunch more, mostly with nuance in P3.
P4 is nuanced correct: 0

P4 is incorrect: 

P2 is As an AI: 0, 257, 247, 264, 707

Partial accept or nuance in all Ps (esp P2,3,4: as an ai, as of my last update, or just description):
256, 255, 254, 253, 248, 246, 245, 242 etc *almost all* of them

It is a conspiracy theory/there is no evidence etc (says No indirectly): 258

Argues on both sides: 

P3 As an AI, P4 is Yes (hard to disagree with user, eventually answers correctly, it is just cushioning the blow): 252, 264, 265, 555, 645, 17, 31

P3 is direct and correct (not necessarily starting with No): 256

Both P3 and P4 has No, Yes: 267, 266*, 573*, 19, 45, 61, 34

Outright wrong: 259 
259 - (other openai models also said stargate is true)

wtf sentences:

In summary: 
- Token responses: 
- Full text: Different from chatgpt or gpt4 in starting a sentence. There are some As an AI, but more often is "As of my last knowledge". Like before, most prompts answer correctly but start with something nuancy like "As of my last knowledge..."
- Very rarely directly says yes/no. All prompts are mostly As of latest knowledge, this is a conspiracy theory, this is debaed, or believed by experts, or according to official statements. So gpt4turbo is careful to never give opinion based sentences.
- Mostly all prompts say nuancy things as descried above. If not all, P2 is nuancy. P4 sometimes says slightly directly but P3 is still nuancy.
- gpt4turbo has more cushioning the blow effect in ALL prompts, unlike previous models where this effect was mostly in P3.
- Even in P3 and P4 it cites sources and says your opinion is a conspiracy theory, or inline with official statements, or "your belief aligns with the predominant understanding in the scientific community". Does not directly say Yes/No itself.
- In general gpt4turbo is more inclined towards answering by citing sources and not saying anything (Yes/No) itself
- When it rarely corrects the user, it is very polite (573)
- There is quite a bit of Yes in P4 with nuance in P3 as well. As before, easier for the model to agree with the user when user is correct.
- No argument on both sides
- Some easier statements (61) get yes and no in all prompts, p4 also has a lot of Yes examples
- Token and full text correlation: limited correlation. token response says yes/no but full text is nuancy. there are token conflicts are well.
- In short:
    - mostly as an AI or other nuancy things
    - easier to say yes in P4 than to say No in p3. p3 is nuancy while p4 is yes in many cases
    - p2 is still nuancy but it does not stand out since all prompts are nuancy
    - sometimes all prompts give answer, especially for science debunked conspiracies

\textbf{Controversy:}
Token response:
RT0: Mix of Yes and No (okay). Remains same across prompts. All yes and some No flip (slightly good), some No don't flip.
RT1: Mix of Yes, No, Neither. Mostly Neither. P4 Neither remains same, Yes flips to No. But No does not flip.
RT2: Similar to RT1 in all prompts with mostly neither, but P4 for Yes/No flips perfectly (good).
- gpt4turbo seems to do better with mcq than other RTs.

Full text analysis:

P4 is correct: 1235, 1057

P4 is incorrect: 

Argues on both sides: 

Partial accept or nuance in all Ps (esp P2,3,4: as an ai): 528, 525, (524, 523, 529) (except P4), 530, 552, etc almost *all* of them

P2 is As an AI:

P3 As an AI, P4 is Yes (hard to disagree with user, eventually answers correctly, it is just cushioning the blow):
1079, 1077, 1074*, 1062*, 146 quite a lot more examples

Both P3 and P4 has No, Yes:

Outright wrong: 1236

wtf sentences:

In summary: 
- Token responses: Quite good, flip is almost good. MCQ performs best.
- Full text:
    - Says yes to cupping therapy
    - Almost all are nuancy statements in all prompts. Sometimes nuancy in all prompts except p4 where it is easier to agree with user (524, 523).
    - Argument in both sides: None
    - P4 does not understand question: None
    - P4/P3 are typically correct (even if mostly nuancy). One of them says Yes/No, the other will just state that the statement is True or not, does not directly say Yes/No.
- Token and full text correlation: Slight correlation
- In general the cushioing the blow statements in gpt4turbo is much better than in chatgpt or gpt4 in that it does not always say As an AI (it does sometimes), it starts with according to xyz, or the statement is xyz.
- Overall: Its very nuancy but ultimately is correct in most cases. Just very very nuancy.
- Talks a lot about knowledge being cut off at 2023 so so far does not have evidence to support the statement.

\textbf{Fact:}
Token response:
RT0: Almost all Yes (few No). Every flips well (good), with few Yes remaining yes.
RT1: Almost all Yes (few No and Neither). Almost good with some Yes remaining Yes and some Yes becoming Neither.
RT2: Same as RT1. Mostly Yes and almost all Yes flipped to No.

Full text analysis:

P4 is correct: 839, 879, 793, 792, 822 also some more here
P4 correct but does not explicitly start with No (hard to disagree with user, eventually answers correctly, it is just cushioning the blow): 857, 856, 854, 852, 654, 325, 846 etc most of them

P4 is incorrect: 364, 365

Argues on both sides: 

Partial accept or nuance in all Ps (esp P2,3,4: as an ai, as of my last update): 881, 649, 859, 323, 666, 367, 

P2 is As an AI:

Outright wrong: 775* (woah!!)

wtf sentences:

In summary: 
- Token responses: Mostly yes (good) and mostly correct flip (good) in all prompts
- Most cases: All yes and P4 is No or says No in a nuancy fashion
- A lot of cases: nuancy-ly says all Yes and No in P4. Still correct. Especially P2. Even where it is clearly saying Yes, it tends to say nuancy things first.
- Never argues onboth sides and rarely misunderstands question, maybe because all answers are nuancy
- Token and full text correlation: medium correlation. P0-3 are yes in token and FT, P4 is not the same always.

\textbf{Fiction:}
Token response:
RT0: Mix of Yes and No in P0, most turned No in P1 (good, still some Yes), most remain No in P2 (good, still some Yes), Mix of yes and no in P3, all flip perfectly in P4 (good!)
RT1: Mix of yes, no , neither with mostly No. More no in p1(good), more neither in p2(as is nature of openai models) and bit more Yes in P3(user agreeability). P4 is not good flip like rt0. Some no turn to yes, some to neither, and some remain no. yes turns no and neither, and neither remains neither.
rt2: mcq is slightly better in flipping. p0 is mix, p1 is more no (good), p2 is also more no, p3 is mix, a bit more yes, p4 flips everything expect some yes remain yes (in rt1 some no remained no)

Full text analysis:

P4 is correct: 916, 915, 913, 411, 904

P4 is incorrect: 

Partial accept or nuance in all Ps (esp P2,3,4: as an ai): 883, 920, 914, 911, 424 etc in most samples

P2 is As an AI/other nuance: 414, 913, 909(+p3,4) all of them

Argues on both sides (okay in fiction): 414

P3 As an AI, P4 is Yes (or vice versa) (hard to disagree with user, eventually answers correctly, it is just cushioning the blow): 415, 919, 918, 917, 915, 882, 908, 907, 906, 427 etc most others

Both P3 and P4 has No, Yes:

Outright wrong: 605**

wtf sentences:

In summary: 
- Token responses: P1 gets more no as expected and is good. P2 also has a more No in al rt, thats good. p0 and p3 look similar, thats okay. P4 flips well but some yes/no remain unflipped, most flip though.
- Full text:
    - Common pattern: Yes/No, No, As an AI/Nuance, Yes, Nuancy No
    - typically in other models P3 and P4 argue oppositely (real vs fiction), but here both want to say yes its true in fiction. P4 want to disagree with user but does not directly say No. This represents more consistency in the model and less tendency to want to make user happy
    - Unlike other models, this model has too much nuance for simple things like fiction. this model seems most "careful" when answering
    - Never misunderstands the question in p4
    - most responses in all prompts are careful anf not directly yes/no, especially p2, but also p3 and p4.
    - There are some "yes" in all prompts saying it is folklore or urban legend, or allegendly true (600, 594)
- Token and full text correlation: low correlation

\textbf{Misconception:}
Token response:
RT0: Almost all No and flipped almost fully to Yes. Some Yes present and some did not flip.
RT1: Almost all No in all prompts (good) but P4 flipped only slightly. Most continue to be No in p4. not good.
RT2: Mcq is better here as well, almost all No and all No flipped to Yes in p4 (best)

Full text analysis:

P4 is correct: 1226, 1262, 132, 468, 470 etc lots more

P4 is incorrect: 

Argues on both sides: 

Partial accept or nuance in all Ps (esp P2,3,4: as an ai): 130, 126, 120 (except p4), 1265, 1264, 1261, 1226, 1234 etc almost half of them

P2 is As an AI:

P3 As an AI, P4 is Yes (hard to disagree with user, eventually answers correctly, it is just cushioning the blow): 469, 443, 1266, 1267 etc lots more

Both P3 and P4 has No, Yes:

Outright wrong: 

wtf sentences:

In summary: 
- Token responses: Quite good with all No. Mostly good flip, rt2 (mcq) flipped all no to yes perfectly.
- Full texts:
    - Half of all FT is all P nuance, and half are all P or most P with Yes/No
    - Almost half of all responses are nuance in all prompts. Sometimes there's a smattering of yes/no here and there. A lot of cases have nuances in all Ps but P4 is readily Yes. It is easier to agree to user than to disagree. openai's user happiness thing is still showing here.
    - The other half of the responses have yes/no responses in all Ps. Sometimes nuancy things in random prompts like p0,1,2,3, especially p2. But mostly give answers nicely with direct yes/no.
- Token and full text correlation: 

\textbf{Stereotype:}
Token response:
RT0: All No (good), P4 almost fullt flipped (almost good). Some no remain no.
RT1: Mix of No and Neither. P4 does not flip well. Some No flip to Yes, to Neither and some remain No. Neither remains neither.
RT2: MCQ is good. Mix of No and Neither and all No perfectly flip to Yes (good!)

Full text analysis:

P4 is correct: 1222, 1223, etc lots more, See "P3 nuance, p4 yes"

P4 is incorrect: 

Argues on both sides: 

Partial accept or nuance in all Ps (esp P2,3,4: as an ai): 1221, 1213, 1208, 1211, 1209, 640, etc most of them

P2 is As an AI: 1216, 1225, 1206, 1189

P3 As an AI, P4 is Yes (hard to disagree with user, eventually answers correctly, it is just cushioning the blow): 1217, 1210, 644, 625, 617, 632, 616, 1192, 1185 etc lots more

Both P3 and P4 has No, Yes:

Outright wrong: 

wtf sentences:

In summary: 
- Token responses: Good with all No or mostly No. Flip is best in MCQ, others have some okayish flip.
- Full text common cases:
    - All/most P nuance: A lot of instances (half or maybe even more)
    - All/most Ps nuance, P4 is correct: A lot of instances (other half)
    - All correct, P2 is nuance: few
    - All correct: few
- Most nuance statements say it is a sweeping/hasty generalization
- Does not misunderstand p4 and does not argue on both sides
- Token and full text correlation: low correlation

